Sportify: Question Answering with Embedded Visualizations and Personified Narratives for Sports Video

As basketball's popularity surges, fans often find themselves confused and overwhelmed by the rapid game pace and complexity. Basketball tactics, involving a complex series of actions, require substantial knowledge to be fully understood. This complexity leads to a need for additional information and explanation, which can distract fans from the game. To tackle these challenges, we present Sportify, a Visual Question Answering system that integrates narratives and embedded visualization for demystifying basketball tactical questions, aiding fans in understanding various game aspects. We propose three novel action visualizations (i.e., Pass, Cut, and Screen) to demonstrate critical action sequences. To explain the reasoning and logic behind players' actions, we leverage a large-language model (LLM) to generate narratives. We adopt a storytelling approach for complex scenarios from both first and third-person perspectives, integrating action visualizations. We evaluated Sportify with basketball fans to investigate its impact on understanding of tactics, and how different personal perspectives of narratives impact the understanding of complex tactic with action visualizations. Our evaluation with basketball fans demonstrates Sportify's capability to deepen tactical insights and amplify the viewing experience. Furthermore, third-person narration assists people in getting in-depth game explanations while first-person narration enhances fans' game engagement

==> README <==
Created by Torsten Moeller, April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016
modified by Cagatay Turkay and Soumya Dutta, September 2019
modified by Cody Dunne, January and March 2023

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used with an established LaTeX environment by calling pdfLaTeX or LaTex. For online collaborative editing or without a local LaTeX installation, one option is to use https://www.overleaf.com/. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Unix-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)


==> sections/backup/1intro_v1.tex <==
%% Sports games, esp multiple players sports, such as basketball,
% In recent years, basketball has significantly grown in popularity, capturing the attention of millions of enthusiasts around the globe. 
% This surge in interest has attracted a diverse audience, including new and casual fans who, 
% despite their enthusiasm for the game, often find its intricacies and strategies challenging to comprehend. 
% The complexity of the sport, combined with the vast amount of data generated through matches, presents a unique challenge: making the game accessible and understandable to this burgeoning fan base~\cite{}.

Sports have significantly grown in popularity, capturing the attention of millions of fans around the world. 
Especially, basketball is one of the most popular sports, boasting 400 million fans in the world \cite{popularSports}. Even the NBA Finals garnered a peak audience of 17 million fans \cite{nbaviewership}. Despite the widespread interests in basketball, many fans are confused and overwhelmed while watching basketball videos, due to by the rapid game pace and complexity \cite{chen2023iball, lin2022quest}. Since the commentary does not cover all the information they need, the fans seek more addition information to understand the games and keep up with the players' performance and statistics such as shooting percentages. The most challenging aspect is to comprehend the strategic and in-game decisions,  which involves a complex series of actions such as screen, pass, cut, and shoot \cite{sicilia2019deephoops}, requiring significant knowledge to be fully understood for fans. Based on these actions, the teams maximize the chances of scoring with in a range of offensive tactics \cite{kohli2015optimal, singh2023optimizing, mcintyre2016recognizing}, as players decide to either shoot or distribute the ball to teammates \cite{skinner2017optimal}. Comprehending these strategy and in-game decisions not only enhances the watching experiences but also deepens the enjoyment of the game. 

Previous research has explored to bridge this gap by leveraging the power of \emph{embedded visualizations}~\cite{willett2016embedded}.  These visualizations integrate data directly within actual game videos in some commercial tools \cite{secondspectrum, courtvision, vizlibero} and research \cite{chen2021augmenting, chen2022sporthesia, chen2023iball, lin2022quest}, creating a term as \emph{augmented sports videos}. This integration allows fans to access important information seamlessly without detracting from the action, enhancing the watching experience by providing insights directly within the context of the ongoing game.  Despite the utility of these augmented sports videos, existing systems have largely been limited to deploying predefined visualizations. For instance, they highlight a player's offensive abilities or trace their trajectories across the court, offering only a static level of insight into the game's dynamics \cite{chen2023iball, lin2022quest}. However, these approaches do not properly support viewers in exploring the game's intricate questions to their personal curiosities. Current offerings are insufficient for the fans, especially when viewers aim to understand broader strategic aspects like a team's offensive tactics \cite{lin2022quest}. The previous works lack the flexibility to dynamically generate responses to complex from users' queries on-the-fly. This limitation highlights a significant gap in the interactive and personalized dimensions of sports viewing, preventing fans from engaging in a deeper exploration of the game to uncover answers to their specific, intriguing questions.

In this paper, we implement a novel Visual Question Answering (VQA) system, \ourtool (\autoref{fig:teaser}), that integrates narratives and embedded visualization for explaining basketball strategies and in-game decision-making questions, aiding fans in understanding various game aspects.
The design of \ourtool is based on three design requirements 1) answering complex questions, 2) explaining strategic and in-game decision questions, and 3) storytelling combining narrative and visualization.
These considerations allow the fans to actively interact with our tool by asking not only simple stats-based questions like players' performance but also complex questions regarding strategic and in-game decisions as \textbf{in the form of augmented sports videos}. 
To explain the strategic questions, we propose three new action visualizations (i.e., Pass, Cut, and Screen) to demonstrate the important action sequences.
The \ourtool extracts the actions by utilizing the coordinates and bounding boxes of players and ball through computer vision pipeline, and a K-Nearest Neighbors (KNN) classifies tactic based on the coordinates. 
By utilizing these extracted textual information, we leverage a large-language model (LLM) to generate narratives to support logic-behind players' actions. 
Our approach incorporates visual and narrative elements in a unique storytelling format, utilizing a \textbf{first-person perspective} for explanation, to enhance comprehension of complex queries.  
This integration of embedded visualization and narrative storytelling ensures that insights are not only accessible but also engaging. 
By enabling this level of interaction and penalization, our VQA system transforms passive viewing into an active exploration of the sport, providing a deeper understanding and engagement among fans.
We conducted two user studies (i.e., a comparative study and a exploratory study) with basketball fans to investigate the impact on the understanding of strategies  and in-game decisions.
We compare three different conditions and two different personal perspective of narratives to explore how different personal perspectives of narratives affect the comprehension of complex strategy with action visualizations. 
The exploratory results demonstrate that \ourtool helps users understand strategic and in-game decisions questions, and enhances user engagement and experience compared to existing tactic explanation videos. 
Furthermore, third-person narration assists people in getting in-depth game explanations while first-person narration enhances fans’ game engagement.

% Our finding is that the QA system with visual interaction helps users understand strategy questions and more engagement user experience.
% We adopt a storytelling approach for complex scenarios from both first and third-person perspectives, integrating action visualizations. 

% The \ourtool utilizes the coordinates and bounding boxes of players and ball.  

% First, it dynamically generates \textbf{answers in the form of augmented sports videos} with embedded visualizations, meticulously crafted to address the user's particular question. 

% Secondly, our approach incorporates visual and narrative elements in a unique storytelling format, utilizing a \textbf{first-person perspective} for explanation, to enhance comprehension of complex queries.  

% This integration of embedded visualization and narrative storytelling ensures that insights are not only accessible but also engaging. 

% By enabling this level of interaction and penalization, our VQA system transforms passive viewing into an active exploration of the sport, fostering a deeper understanding and engagement among fans.
% Results here.
% Specifically, our VQA system xxxx.

In summary, our contributions are as follow: 1) the implementation and design of a novel VQA system for answering strategic and in-game decisions, 2) three novel visualizations such as Cut, Screen, and Pass, integrating the narratives such as third and first person perspectives to provide a storytelling experience that enhances the engagement for fans, and 3) two user studies that evaluate three different conditions with two different person perspectives, and the usability of \ourtool comparing to existing strategy explanation videos.

% Contribution: 1. implement and design system 2. evaluate the system 3. design driven
%     - answer how to explain tactic visually in video - design framework
%     - dev system VQA - support design 
%     - evaluation

% This method acknowledges that data visualization in sports analytics, especially when addressing sophisticated strategic concepts, demands more than just presenting data; it requires effective narration to bridge the gap between raw data and comprehensible insights.

% To achieve this, we propose a novel narrative technique: a first-person perspective data visualization narrative. This perspective places the viewer directly in the shoes of players or key decision-makers, offering a unique vantage point that enhances the storytelling aspect of data visualization. By doing so, we not only provide answers to specific questions but also enrich the viewer's comprehension and engagement through a more immersive experience. This approach leverages the power of storytelling to make complex data and strategies accessible and engaging, thereby addressing the previously identified gap in interactive sports analytics.



%%%%

% We implement a QA system to support different types of question and especially focus on strategy and in-game questions, which are complex scenarios. To explain the question, we support visual and narrative elements like storytelling. The data visualization is more complex than other storytelling, which requires effective narration. We propose 1st person perspective data visualization narrative.



% passive vs active
% 1st vs 3rd - contribution 
% validate emmersive
% how to 1st and 3rd (embeddev visualization)

==> sections/backup/1intro_v2.tex <==
%% Sports games, esp multiple players sports, such as basketball,
% In recent years, basketball has significantly grown in popularity, capturing the attention of millions of enthusiasts around the globe. 
% This surge in interest has attracted a diverse audience, including new and casual fans who, 
% despite their enthusiasm for the game, often find its intricacies and strategies challenging to comprehend. 
% The complexity of the sport, combined with the vast amount of data generated through matches, presents a unique challenge: making the game accessible and understandable to this burgeoning fan base~\cite{}.

% Sports have significantly grown in popularity, capturing the attention of millions of fans around the world. 
% Especially, 

Basketball attracts 400 millions fans worldwide~\cite{popularSports}, with the NBA Finals alone drawing a peak audience of 17 million~\cite{nbaviewership}. 
% This passion underscores the sport's standing as a global phenomenon. 
Despite widespread interest in basketball, the rapid pace and intricate dynamics of the basketball plays often leave fans confused and eager for a deeper understanding of the game~\cite{chen2023iball, lin2022quest}.
%However, amidst the exhilaration lies a challenge: the rapid pace and intricate dynamics of basketball often leave fans bewildered and thirsting for a deeper understanding of the game~\cite{chen2023iball, lin2022quest}. 
While commentary provides some insights, 
it lacks in providing the abundance of information fans desire, from player performance metrics to complex strategic decisions. 
Particularly, understanding the tactics represents a significant but challenging task. 
%It involves a multifaceted series of actions—screening, passing, cutting, and shooting—that requires not only significant knowledge but also an appreciation for the subtleties of the sport~\cite{sicilia2019deephoops}.
It involves a multifaceted series of actions—screening, passing, cutting, and shooting—that requires significant knowledge to be fully understood~\cite{sicilia2019deephoops}.
These tactics are crucial in maximizing scoring opportunities, from single plays to team-wide strategies~\cite{kohli2015optimal, singh2023optimizing, mcintyre2016recognizing}.
Players constantly make split-second decisions to either take the shot or distribute the ball, optimizing their team's offensive tactics~\cite{skinner2017optimal}. 
%the teams maximize their scoring opportunities through a variety of offensive strategies \cite{kohli2015optimal, singh2023optimizing, mcintyre2016recognizing}, with players choosing to either take shots or pass the ball to their teammates \cite{skinner2017optimal}.
A deeper comprehension of these tactics not only enhances the watching experience but also significantly deepens fans' enjoyment and engagement of the game.

Recent efforts in bridging the knowledge gap for fans have embraced the concept of \emph{embedded visualizations}~\cite{willett2016embedded}. 
These visualizations seamlessly integrate data into actual scenes,
enriching the watching experience by embedding insights within the physical context of the match.
Therefore, 
embedded visualizations have been widely used by both commercial ~\cite{secondspectrum, courtvision, vizlibero} and research systems~\cite{chen2021augmenting, chen2022sporthesia, chen2023iball, lin2022quest} to create \emph{augmented sports videos}.
Current augmented sports video products and studies are innovative but limited to deploying predefined visualizations, 
offering a fixed set of insights for the game's inherently dynamic character~\cite{chen2023iball, lin2022quest}. 
Such limitations hinder fans' ability to engage with more detailed strategic elements of game play, restricting the exploration of personal interests or inquiries. 
Notably, these tools lack interactive features that would allow fans to investigate the game's strategic dimensions, a limitation that restricts personalized engagement and understanding of complex tactics~\cite{lin2022quest}.
This reveals the requirement for advanced game watching systems that enable fans to dynamically explore and query game strategies.

In this paper, we develop a novel Visual Question Answering (VQA) system, \ourtool (\autoref{fig:teaser}), 
which integrates embedded visualization and personified narratives to explain basketball strategies and in-game decisions, 
thereby assisting fans in understanding various game aspects.
The design of \ourtool is guided by three design requirements: 
1) active interactions to answer users' questions, 
2) explaining strategic and in-game decision questions, 
and 3) storytelling combining narrative and visualization.
These considerations allow the fans to actively interact with our tool by asking not only simple stats-based questions (e.g., players' performance) but also complex questions regarding strategic and in-game decisions.

% \textbf{in the form of augmented sports videos}. 
To explain the strategic questions, we propose three new action visualizations (i.e., Pass, Cut, and Screen)  that illustrate key action sequences critical to understanding basketball strategies.
% for demonstrating the important action sequences.
% \ourtool extracts these actions by utilizing the coordinates and bounding boxes of players and ball through computer vision pipeline, and a K-Nearest Neighbors (KNN) classifies tactic based on the coordinates. 
% By utilizing these extracted textual information, we leverage a large-language model (LLM) to generate narratives to support logic-behind players' actions. 
\ourtool leverages a computer vision pipeline to identify these actions, utilizing player and ball coordinates and bounding boxes. 
A K-Nearest Neighbors (KNN) algorithm classifies tactics based on these coordinates. The results are subsequently used to generate insightful narratives about the logic behind players' actions by using a large language model (LLM).
Moreover, our approach integrates visual elements with narratives in a distinctive storytelling format, adopting a \textbf{first-person perspective} for explanations. 
This approach not only facilitates comprehension of complex questions but also engages users by embedding insights within an interactive and attracting narrative framework.
Through this integration of embedded visualization and narrative, 
\ourtool transforms passive viewing into an active exploration experiences, offering a deeper understanding and engagement with the game.

% incorporates visual and narrative elements in a unique storytelling format, utilizing a \textbf{first-person perspective} for explanation, to enhance comprehension of complex queries.  
% This integration of embedded visualization and narrative storytelling ensures that insights are not only accessible but also engaging. 
% By enabling this level of interaction and penalization, our VQA system transforms passive watching into an active exploration of the sport, providing a deeper understanding and engagement among fans.

We conducted two user studies (i.e., a comparative study and a exploratory study) with basketball fans to investigate the impact on understanding of strategies and in-game decisions.
We compare three different conditions and two narrative perspective to explore their impacts on the comprehension of basketball strategy.
% with action visualizations. 
The results demonstrate that \ourtool helps users understand strategic and in-game decisions better, 
and enhances user engagement and experience compared to existing tactic explanation videos. 
Furthermore, third-person perspective narration assists people in getting in-depth game explanations while first-person narration enhances fans' game fan and engagement.

In summary, our contributions are as follow: 1) the implementation and design of a novel VQA system for answering strategic and in-game decisions, 2) three novel visualizations such as Cut, Screen, and Pass, integrating the narratives such as third and first person perspectives to provide a storytelling experience that enhances the engagement for fans, and 3) two user studies that evaluate three different conditions with two different person perspectives, and the usability of \ourtool comparing to existing strategy explanation videos.

% Our finding is that the QA system with visual interaction helps users understand strategy questions and more engagement user experience.
% We adopt a storytelling approach for complex scenarios from both first and third-person perspectives, integrating action visualizations. 

% The \ourtool utilizes the coordinates and bounding boxes of players and ball.  

% First, it dynamically generates \textbf{answers in the form of augmented sports videos} with embedded visualizations, meticulously crafted to address the user's particular question. 

% Secondly, our approach incorporates visual and narrative elements in a unique storytelling format, utilizing a \textbf{first-person perspective} for explanation, to enhance comprehension of complex queries.  

% This integration of embedded visualization and narrative storytelling ensures that insights are not only accessible but also engaging. 

% By enabling this level of interaction and penalization, our VQA system transforms passive viewing into an active exploration of the sport, fostering a deeper understanding and engagement among fans.
% Results here.
% Specifically, our VQA system xxxx.



% Contribution: 1. implement and design system 2. evaluate the system 3. design driven
%     - answer how to explain tactic visually in video - design framework
%     - dev system VQA - support design 
%     - evaluation

% This method acknowledges that data visualization in sports analytics, especially when addressing sophisticated strategic concepts, demands more than just presenting data; it requires effective narration to bridge the gap between raw data and comprehensible insights.

% To achieve this, we propose a novel narrative technique: a first-person perspective data visualization narrative. This perspective places the viewer directly in the shoes of players or key decision-makers, offering a unique vantage point that enhances the storytelling aspect of data visualization. By doing so, we not only provide answers to specific questions but also enrich the viewer's comprehension and engagement through a more immersive experience. This approach leverages the power of storytelling to make complex data and strategies accessible and engaging, thereby addressing the previously identified gap in interactive sports analytics.



%%%%

% We implement a QA system to support different types of question and especially focus on strategy and in-game questions, which are complex scenarios. To explain the question, we support visual and narrative elements like storytelling. The data visualization is more complex than other storytelling, which requires effective narration. We propose 1st person perspective data visualization narrative.



% passive vs active
% 1st vs 3rd - contribution 
% validate emmersive
% how to 1st and 3rd (embeddev visualization)

==> sections/backup/1intro_v3.tex <==
Basketball attracts 400 millions fans worldwide~\cite{popularSports}, with the NBA Finals alone drawing a peak audience of 17 million~\cite{nbaviewership}. 
Despite widespread interest in basketball, the rapid pace and intricate dynamics of the basketball plays often leave fans confused and eager for a deeper understanding of the game~\cite{chen2023iball, lin2022quest}.
Commentary, while helpful, often lacks in providing the abundance of information fans desire, from player performance metrics to complex tactical decisions. 
Particularly, understanding the tactics represents a significant but challenging task. 
It involves a multifaceted series of actions—screening, passing, cutting, and shooting—that requires significant knowledge to be fully understood~\cite{sicilia2019deephoops}.
These tactics are crucial in maximizing scoring opportunities, from single plays to team-wide tactics~\cite{kohli2015optimal, singh2023optimizing, mcintyre2016recognizing}.
Players constantly make split-second decisions to either take the shot or distribute the ball, optimizing their team's offensive tactics~\cite{skinner2017optimal}. 
A deeper comprehension of these tactics not only enhances the watching experience but also deepens fans' engagement of the game.

Recent efforts in bridging the knowledge gap for fans have embraced the concept of \emph{embedded visualizations}~\cite{willett2016embedded}. 
These visualizations 
enrich the watching experience by seamlessly integrating 
data insights within the physical context of the game.
Therefore, 
embedded visualizations have been widely used by both commercial ~\cite{secondspectrum, courtvision, vizlibero} and research systems~\cite{chen2021augmenting, chen2022sporthesia, chen2023iball, lin2022quest} to create \emph{augmented sports videos}.
Current augmented sports video products and systems are innovative but limited to deploying predefined visualizations, 
offering a fixed set of insights for the game's inherently dynamic character~\cite{chen2023iball, lin2022quest}. 
% Such limitations hinder fans' ability to engage with more detailed strategic elements of game play, restricting the exploration of personal interests or inquiries. 
\zt{find somewhere to clearly define ``Tactics = a serious of actions''}
Notably, these tools lack interactive features that would allow fans to investigate the game's tactical dimensions, a limitation that restricts personalized engagement and understanding of complex tactics~\cite{lin2022quest}.
This reveals the requirement for advanced game watching systems that enable fans to dynamically explore and query game tactics.

In this paper, we develop a novel Visual Question Answering (VQA) system, \ourtool{} (\autoref{fig:teaser}), 
which integrates embedded visualization and personified narratives to explain basketball tactics, 
thereby assisting fans in understanding various game aspects.
The design of \ourtool \space is guided by three design considerations: 
1) explaining tactics with grounded video data,
% active interactions to answer users' questions, 
2) explaining tactics with narratives, 
and 3) explaining tactics using embedded visualizations.
These considerations allow the fans to actively interact with our tool by asking not only simple stats-based questions (e.g., players' performance) but also complex questions regarding tactic and in-game decisions.

% \textbf{in the form of augmented sports videos}. 
To explain questions about tactics and in-game decisions, 
\ourtool{} \space leverages a computer vision pipeline to identify three actions (i.e., Pass, Cut, and Screen),
which are critical to understanding basketball tactics,
by utilizing player and ball coordinates and bounding boxes. 
A K-Nearest Neighbors (KNN) algorithm classifies the tactics based on the players' coordinates. 
The results are subsequently used to generate answers 
about the logic behind players' actions 
by using a large language model (LLM).
To present the answers, 
we propose three new action visualizations (i.e., Pass, Cut, and Screen) and two personified narratives (i.e., \textbf{first-person} and \textbf{third-person} perspectives), explaining the answers in a storytelling format.
% for demonstrating the important action sequences.
% \ourtool extracts these actions by utilizing the coordinates and bounding boxes of players and ball through computer vision pipeline, and a K-Nearest Neighbors (KNN) classifies tactic based on the coordinates. 
% By utilizing these extracted textual information, we leverage a large-language model (LLM) to generate narratives to support logic-behind players' actions. 
% This approach not only facilitates comprehension of strategy questions but also engages users by embedding insights within an interactive and attracting narrative framework.
Through the integration of embedded visualization and narrative, 
\ourtool{} transforms passive viewing into an active exploration experiences, offering a deeper understanding and engagement with the game.

% incorporates visual and narrative elements in a unique storytelling format, utilizing a \textbf{first-person perspective} for explanation, to enhance comprehension of complex queries.  
% This integration of embedded visualization and narrative storytelling ensures that insights are not only accessible but also engaging. 
% By enabling this level of interaction and penalization, our VQA system transforms passive watching into an active exploration of the sport, providing a deeper understanding and engagement among fans.

We conducted two user studies (i.e., a comparative study and a exploratory study) with basketball fans to investigate the impact on understanding of tactics and in-game decisions.
We compare three different conditions and two narrative perspective to explore their impacts on the comprehension of basketball tactic.
% with action visualizations. 
The results demonstrate that \ourtool{} helps users understand tactics and in-game decisions better, 
and enhances user engagement and experience compared to existing tactic explanation videos. 
Furthermore, third-person perspective narration assists people in getting in-depth game explanations while first-person narration enhances fans' game fan and engagement.

In summary, our contributions are as follow: 1) the implementation and design of a novel VQA system for answering tactics and in-game decisions, 2) three novel visualizations such as Cut, Screen, and Pass, integrating the personified narratives (i.e., first or thrid person perspective) to provide a storytelling experience that enhances the engagement for fans, and 3) two user studies that evaluate three different conditions with the two personified perspectives texts, and the usability of \ourtool{} comparing to existing tactic explanation videos.

% Our finding is that the QA system with visual interaction helps users understand strategy questions and more engagement user experience.
% We adopt a storytelling approach for complex scenarios from both first and third-person perspectives, integrating action visualizations. 

% The \ourtool utilizes the coordinates and bounding boxes of players and ball.  

% First, it dynamically generates \textbf{answers in the form of augmented sports videos} with embedded visualizations, meticulously crafted to address the user's particular question. 

% Secondly, our approach incorporates visual and narrative elements in a unique storytelling format, utilizing a \textbf{first-person perspective} for explanation, to enhance comprehension of complex queries.  

% This integration of embedded visualization and narrative storytelling ensures that insights are not only accessible but also engaging. 

% By enabling this level of interaction and penalization, our VQA system transforms passive viewing into an active exploration of the sport, fostering a deeper understanding and engagement among fans.
% Results here.
% Specifically, our VQA system xxxx.



% Contribution: 1. implement and design system 2. evaluate the system 3. design driven
%     - answer how to explain tactic visually in video - design framework
%     - dev system VQA - support design 
%     - evaluation

% This method acknowledges that data visualization in sports analytics, especially when addressing sophisticated strategic concepts, demands more than just presenting data; it requires effective narration to bridge the gap between raw data and comprehensible insights.

% To achieve this, we propose a novel narrative technique: a first-person perspective data visualization narrative. This perspective places the viewer directly in the shoes of players or key decision-makers, offering a unique vantage point that enhances the storytelling aspect of data visualization. By doing so, we not only provide answers to specific questions but also enrich the viewer's comprehension and engagement through a more immersive experience. This approach leverages the power of storytelling to make complex data and strategies accessible and engaging, thereby addressing the previously identified gap in interactive sports analytics.



%%%%

% We implement a QA system to support different types of question and especially focus on strategy and in-game questions, which are complex scenarios. To explain the question, we support visual and narrative elements like storytelling. The data visualization is more complex than other storytelling, which requires effective narration. We propose 1st person perspective data visualization narrative.



% passive vs active
% 1st vs 3rd - contribution 
% validate emmersive
% how to 1st and 3rd (embeddev visualization)

==> sections/backup/3design_v1.tex <==
\begin{figure*}[ht]
\centering
\includegraphics[width=1.0\textwidth]{figs/system.png}
\caption{The pipeline of answering and explaining not only strategic and in-game decision questions but also performance based questions. The data pipeline (A) takes video and utilize CV pipeline to extract players' position and bounding box, and ball position. Those outputs are taken to action detection (B) and tactic classifier (C) to make high-level textual information. The players' coordinates and responses from LLM visualize in the video. For the performance questions are taken by LLM to retrieve data and answer as a form of text.}
\label{fig:system}
\end{figure*}

\section{Design Requirements}

We detail the design considerations for \ourtoolnospace, 
which are informed by our extensive experience in developing visualization tools for game watching over several years.

% We outline the design considerations of \ourtoolnospace,
% which stem from our multiple years' experiences on developing visualizations tools for game watching.
% analysis of prior research. 

% to support active game watching experiences.

% , which features 
% active interactions to respond to users' questions, 
% incorporating embedded visualizations to explain strategic and in-game decision questions through storytelling approach. These requirements stem from our analysis of prior research. 

\vspace{1mm}
\noindent\textbf{R1. Supporting active question asking.}
Due to the complexity of player movements and the game's rapid pace,
basketball fans often find themselves overwhelmed when watching basketball games.
Previous works~\cite{chen2023iball, lin2022quest} identified that audiences frequently had highly personalized questions about the game during the game watching
(e.g., \textit{``check the average stats of three players''} and \textit{``Thunder is missing a lot of 3 pointers''}), and can hardly be covered the a predefined set of embeded visualizations.
Such as gap highlights the needs for more active and personalized interactions beyond passive viewing of statistics-based visualizations. 
% To help the fans, simple visualizations drawing on statistical data, such as shooting percentages and player positioning, are provided in previous work with embedded visualizations~\cite{chen2023iball, lin2022quest}. 

% These previous systems  the main players and the dynamics of ball movement. However, both works 
% Both casual and avid fans frequently require additional data to fully comprehend player performance and team dynamics.
% Often, casual and die-hard fans alike need more additional data to understand and gain further insights into players' performance and teams' metadata. 

To facilitate more personalized game understanding, 
\ourtool should allow users to ask both 
stats-based questions like players' performance and teams' metadata 
and strategic questions such as the tactics and in-game decisions.
To this end, \ourtool features a natural language user interface that allows
users to ask their own questions about the on-going game video. 
% and seamlessly interact with the game views.
% complicated questions tailored to individual needs.
% question-answering interface to allow 
% needs to provide interactions to answer both 

\vspace{1mm}
\noindent\textbf{R2. Explaining tactics and in-game decisions.}
Based on the formative study in prior work~\cite{lin2022quest}, basketball fans are curious and eager to understand the strategies and in-game decisions (e.g., \textit{"the usage of this particular play"} and \textit{"understand the offensive and defensive strategies"}), which requires a breakdown of actions in the gameplay. Yet, prior studies \cite{zhi2020gamebot, lin2022quest, chen2023iball} were not able to answer these intricate questions posed by the fans with embedded visualizations in the game videos. The challenge of explaining strategies and in-game decisions lies in highlighting a series of complex actions and presenting the logic behind player movements. Three fundamental basketball actions, passing, screening, and cutting, were integrated to form various offensive strategies~\cite{sicilia2019deephoops}. Based on this sequence of actions, the team strategically optimizes its shooting opportunities, with players choosing either to take shots or pass to teammates for better chances \cite{kohli2015optimal, singh2023optimizing,skinner2017optimal}. 

To describe the details for strategies and in-game decisions, \ourtool needs to consider three key components, including \textbf{narration} of action sequences to explain the logic, \textbf{embedded visualization} to specify individual actions, and \textbf{animations} to highlight main movement. First, \textbf{narration} is essential for organizing human experience \cite{mayr2018once, schroder2023telling} and describing the causal relationships \cite{choudhry2020once} and the reasons behind players' actions. To achieve comprehensive narration generation for sports strategies, 
we require a powerful LLM that can not only infer the current situation of actions but also deduce the causal relationship between multiple actions. Further, these narratives should also accompany spatiotemporal data visualizations for better understanding, which necessitates appropriate integration during video playback.
% 
Second, \textbf{embedded visualizations} are required to highlight critical actions, i.g., the pass, the screen, and the cut within the game video. For each action, specific considerations are necessary. For a pass, it is essential to clearly indicate the players giving and receiving the pass. In the case of a screen, one player must obstruct another player's movement, and for a cut, the objective is to evade the defense and move into a broader offensive position. Visualization designs are required to depict these actions clearly. Furthermore, \textbf{animations} are essential for visually distinguishing among the complex movements, highlighting key players and actions. 
% 
Therefore, a second design goal of \ourtool is to answer strategies and in-game decisions with the automatic creation of narration, embedded visualization, and animations.
% By further examining these links, we find that narrations and animations of data clips can echo each other by repeating the information conveyed, complement each other by providing additional information, or indirectly link to each other by communicating data contents from different perspectives. Animations and narrations can also work independently to deliver messages.
% Investigating the Role and Interplay of Narrations and Animations in Data Videos

\vspace{1mm}
\noindent\textbf{R3. Presenting explanations with visualization and narrative.}
In order to explain complicated actions, causal relationships, and the reasons behind players' movements, we require a storytelling approach that allows for the effective and intuitive presentation of information through visualization, akin to the experience of watching a film \cite{gershon2001storytelling}. A well-structured story is crucial for simplifying information comprehension, weaving details into a cohesive story rather than presenting information separately.
In addition, effective storytelling requires careful selection of narrative perspective—first, second, or third person—as this choice can significantly influence a player's engagement and immersion in the game. Prior research \cite{chen2021changing} found that a first-person perspective leads to a more immersive reading experience with deeper connection with he narrative, while the third-person viewpoint allows broader reflection on character interactions and their consequences. 
This distinction suggests that different narrative viewpoints may have different effects and require separate design considerations in visual storytelling.

In basketball, the third-person perspective aligns with a commentator's view, offering a broad overview of the game, while the first-person perspective resonates with the individual player's decision-making process. Each perspective offers potential benefits in game understanding.
Meanwhile, each technique encompasses different visualization and narration design considerations. In the first-person perspective, narration needs to be tied to specific subjects in the visualization, while in the third person, the connection between visualizations and narration can be more subtle. 
Thus, it's essential for \ourtool to accommodate various storytelling techniques and incorporate appropriate visualizations to match the chosen narrative method.
% In a basketball game, the third-person perspective refers to the commentator, while the first-person perspective refers to the player. The \textbf{third-person perspective}
%  describes the actions of the players as they are happening, so it does not require any special combination of description and visualization. However, in the case of the \textbf{first-person perspective}, since the player is the subject of the conversation, a narration method combined with visualization is needed. For this reason, we should allow \ourtool to provide different narration methods that are integrated visualization based on different person perspectives.

% \begin{itemize}
% \item previous works answers questions, but indirect and passive way to answer that --> active and direct answer systems.
% \item tactic and strategy question: complex because of multiple players, actions, and in-game decisions --> narratives, visual elements, animations are required.
% Wojtkowski and Wojtkowski [27] further argue that what makes data visualization different from other types of visual storytelling is the complexity of the content that needs to be communicated.
% \item The narrative also important, because 1st and 3rd makes different UX (While in general the 1st person perspective leads to a more immersive reading experience than a 3rd person perspective from paper) --> for more engagement, we build a 1st person perspective visualization? and narrative
% \end{itemize}

==> sections/backup/3design_v2.tex <==
\begin{figure*}[ht]
\centering
\includegraphics[width=1.0\textwidth]{figs/system.png}
\caption{The pipeline efficiently addresses both tactical and performance-based questions. It begins with data processing (A-1), where videos undergo a computer vision (CV) pipeline to identify players' coordinates, bounding boxes, and the ball's location. This information feeds into action detection (A-2) and tactic classification (A-3), generating tactical textual information for the narrative agent (B-1). Player coordinates and LLM responses are visually embedded (C) and displayed in the video (D). Performance-related queries are handled by the LLM, which retrieves data to provide text-based answers (D).}
\label{fig:system}
\end{figure*}

\section{Designing \ourtool{}}
This section first describes the design considerations behind \ourtool{}
and then overviews its three major components.

\subsection{Design Considerations}
Informed by an analysis of previous research~\cite{},
we conceived the design considerations for \ourtool{} as follow:

\para{R1. Supporting active question asking.}
Due to the complexity of player movements and the game's rapid pace,
basketball fans often find themselves overwhelmed when watching basketball games.
Previous works~\cite{chen2023iball, lin2022quest} identified that 
audiences frequently had highly personalized questions about the game during the game watching
(e.g., \textit{``check the average stats of three players''} and \textit{``Thunder is missing a lot of 3 pointers''}), and can hardly be covered the a predefined set of embeded visualizations.
Such as gap highlights the needs for more active and personalized interactions beyond passive viewing of statistics-based visualizations. 

To facilitate more personalized game understanding, 
\ourtool{} should allow users to ask both 
stats-based questions like players' performance and teams' metadata 
and strategic questions such as the tactics and in-game decisions.
To this end, \ourtool{} features a natural language user interface that allows
users to ask their own questions about the on-going game video. 

\para{R2. Explaining tactics.}
Based on the formative study in prior work~\cite{lin2022quest}, basketball fans are curious and eager to understand the tactics (e.g., \textit{``the usage of this particular play''} and \textit{``understand the offensive and defensive tactics''}), which requires a breakdown of actions in the gameplay. Yet, prior studies~\cite{zhi2020gamebot, lin2022quest, chen2023iball} were not able to answer these intricate questions posed by the fans with embedded visualizations in the game videos. 
The challenge of explaining tactics lies in highlighting a series of complex actions and presenting the logic behind player movements. 
Three fundamental basketball actions, \Pass{}, \Screen{}, and \Cut{}, were integrated to form various offensive strategies~\cite{sicilia2019deephoops}. 
Based on this sequence of actions, the team tactically optimizes its shooting opportunities, with players choosing either to take shots or pass to teammates for better chances \cite{kohli2015optimal, singh2023optimizing,skinner2017optimal}. 

To describe the details for tactics, \ourtool{} needs to consider three key components, including \textbf{narration} of action sequences to explain the logic, \textbf{embedded visualization} to specify individual actions, and \textbf{animations} to highlight main movement. 
First, \textbf{narration} is essential for organizing human experience~\cite{mayr2018once, schroder2023telling} and describing the causal relationships \cite{choudhry2020once} and the reasons behind players' actions. To achieve comprehensive narration generation for sports tactics,  we require a powerful LLM that can not only infer the current situation of actions but also deduce the causal relationship between multiple actions. Further, these narratives should also accompany spatiotemporal data visualizations for better understanding, which necessitates appropriate integration during video playback.

Second, \textbf{embedded visualizations} are required to highlight critical actions, i.g., the pass, the screen, and the cut within the game video. For each action, specific considerations are necessary. For a pass, it is essential to clearly indicate the players giving and receiving the pass. In the case of a screen, one player must obstruct another player's movement, and for a cut, the objective is to evade the defense and move into a broader offensive position. Visualization designs are required to depict these actions clearly. Furthermore, \textbf{animations} are essential for visually distinguishing among the complex movements, highlighting key players and actions. 
Therefore, a second design goal of \ourtool{} is to answer tactics and in-game decisions with the automatic creation of narration, embedded visualization, and animations.
% By further examining these links, we find that narrations and animations of data clips can echo each other by repeating the information conveyed, complement each other by providing additional information, or indirectly link to each other by communicating data contents from different perspectives. Animations and narrations can also work independently to deliver messages.
% Investigating the Role and Interplay of Narrations and Animations in Data Videos

\vspace{1mm}
\noindent\textbf{R3. Presenting explanations with visualization and narrative.}
In order to explain complicated actions, causal relationships, and the reasons behind players' movements, we require a storytelling approach that allows for the effective and intuitive presentation of information through visualization, akin to the experience of watching a film \cite{gershon2001storytelling}. A well-structured story is crucial for simplifying information comprehension, weaving details into a cohesive story rather than presenting information separately.
In addition, effective storytelling requires careful selection of narrative perspective—first, second, or third person—as this choice can significantly influence a player's engagement and immersion in the game. Prior research \cite{chen2021changing} found that a first-person perspective leads to a more immersive reading experience with deeper connection with he narrative, while the third-person viewpoint allows broader reflection on character interactions and their consequences. 
This distinction suggests that different narrative viewpoints may have different effects and require separate design considerations in visual storytelling.

In basketball, the third-person perspective aligns with a commentator's view, offering a broad overview of the game, while the first-person perspective resonates with the individual player's decision-making process. Each perspective offers potential benefits in game understanding.
Meanwhile, each technique encompasses different visualization and narration design considerations. In the first-person perspective, narration needs to be tied to specific subjects in the visualization, while in the third person, the connection between visualizations and narration can be more subtle. 
Thus, it's essential for \ourtool{} to accommodate various storytelling techniques and incorporate appropriate visualizations to match the chosen narrative method.
% In a basketball game, the third-person perspective refers to the commentator, while the first-person perspective refers to the player. The \textbf{third-person perspective}
%  describes the actions of the players as they are happening, so it does not require any special combination of description and visualization. However, in the case of the \textbf{first-person perspective}, since the player is the subject of the conversation, a narration method combined with visualization is needed. For this reason, we should allow \ourtool to provide different narration methods that are integrated visualization based on different person perspectives.

% \begin{itemize}
% \item previous works answers questions, but indirect and passive way to answer that --> active and direct answer systems.
% \item tactic and strategy question: complex because of multiple players, actions, and in-game decisions --> narratives, visual elements, animations are required.
% Wojtkowski and Wojtkowski [27] further argue that what makes data visualization different from other types of visual storytelling is the complexity of the content that needs to be communicated.
% \item The narrative also important, because 1st and 3rd makes different UX (While in general the 1st person perspective leads to a more immersive reading experience than a 3rd person perspective from paper) --> for more engagement, we build a 1st person perspective visualization? and narrative
% \end{itemize}

\subsection{System Overview}
\zt{use a paragraph to introduce the overview of the system}
\zt{explain our system consists of three major components and how they connect with each other}

Based on the design requirements analyzed in Section 3, we introduce \ourtool{}, a visual question-answering (VQA) system designed to elucidate complex questions (R1), such as those related to strategy and in-game decisions (R2). This tool combines narrative and visualization techniques for effective storytelling (R3). \ourtool{} consists of two pipeline parts that allow users to ask not only strategic and in-game decision questions but also performance- and stats-based questions.

==> sections/backup/3design_v3.tex <==
\begin{figure*}[ht]
\centering
\includegraphics[width=1.0\textwidth]{figs/system.png}
\caption{The pipeline efficiently addresses both tactical and performance-based questions. It begins with data processing (A-1), where videos undergo a computer vision (CV) pipeline to identify players' coordinates, bounding boxes, and the ball's location. This information feeds into action detection (A-2) and tactic classification (A-3), generating tactical textual information for the narrative agent (B-1). Player coordinates and LLM responses are visually embedded (C) and displayed in the video (D). Performance-related queries are handled by the LLM, which retrieves data to provide text-based answers (D).}
\label{fig:system}
\end{figure*}

\section{Designing \ourtool{}}

% Based on the formative study in prior work~\cite{lin2022quest}, basketball fans are curious and eager to understand the tactics (e.g., \textit{``the usage of this particular play''} and \textit{``understand the offensive and defensive tactics''}), which requires a breakdown of actions in the gameplay. 

% Yet, prior studies~\cite{zhi2020gamebot, lin2022quest, chen2023iball} were not able to answer these intricate questions posed by the fans with embedded visualizations in the game videos. 
% The challenge of explaining tactics lies in highlighting a series of complex actions and presenting the logic behind player movements. 
% Three fundamental basketball actions, \Pass{}, \Screen{}, and \Cut{}, were integrated to form various offensive strategies~\cite{sicilia2019deephoops}. 
% Based on this sequence of actions, the team tactically optimizes its shooting opportunities, with players choosing either to take shots or pass to teammates for better chances \cite{kohli2015optimal, singh2023optimizing,skinner2017optimal}. 

This section first describes the design considerations behind \ourtool{}
and then overviews its three major components.

\subsection{Design Considerations}
Our QA system specifically focuses on questions related to basketball tactics. 
We recognize the potential of leveraging LLMs. 
However, the complexity of accurately explaining tactics in sports analytics demands more than just 
the raw generative power of LLMs.
Specifically, the challenge of answering tactic-related questions 
lies in \emph{explaining a series of complex actions} 
and presenting the logic behind player movements in a \emph{understandable}, \emph{reliable}, and \emph{engaging} manner.
Informed by an analysis of previous research~\cite{},
we conceived the design considerations for \ourtool{} as follow:

% The foundational design considerations of \ourtool{} are guided by the objective of elucidating tactics effectively. Drawing upon insights from prior research, we have developed the following strategic framework:

% Due to the complexity of player movements and the game's rapid pace,
% basketball fans often find themselves overwhelmed when watching basketball games.
% Previous works~\cite{chen2023iball, lin2022quest} identified that 
% audiences frequently had highly personalized questions about the game during the game watching
% (e.g., \textit{``check the average stats of three players''} and \textit{``Thunder is missing a lot of 3 pointers''}), and can hardly be covered the a predefined set of embedded visualizations.
% Such as gap highlights the needs for more active and personalized interactions beyond passive viewing of statistics-based visualizations. 
% To facilitate more personalized game understanding, 
% \ourtool{} should allow users to ask both 
% tactic questions such as the tactics and in-game decisions
% and stats-based questions like players' performance and teams' metadata 
% To this end, \ourtool{} features a natural language user interface that allows
% users to ask their own questions about the on-going game video. 

\para{R1. Explaining Tactics with Narratives.}
Storytelling is fundamental in organizing and conveying human experiences, 
playing a crucial role in how we understand and interpret events~\cite{mayr2018once, schroder2023telling}.
To help users easily understand the tactics employed by teams,
we propose the use of well-structured \emph{narratives} that adhere to a logical sequence. 
This approach not only clarifies the sequence of actions 
but also reveals the underlying reasons and objectives guiding the players' movements~\cite{choudhry2020once}. 
Moreover, the choice of narrative perspective—whether first, second, or third person—also demands careful consideration, as it significantly impacts a viewer's engagement and immersion~\cite{chen2021changing}. 
In basketball, the third-person perspective aligns with a commentator's view, offering a broad overview of the game, while the first-person perspective resonates with the individual player's decision-making process. 
Each perspective offers potential benefits in game understanding.
Finally, it is essential that these narratives are not only presented as plain text 
but organized in a structural format that can be effectively mapped or linked with data visualizations embedded within the video.
% , these narratives should also be able to organized and represented in a structural format,
% so that they can be mapped or connected with data visualizations embedded in the video for better understanding,
% content to facilitates a deeper and more intuitive understanding.
% Such integration facilitates a deeper and more intuitive understanding by ensuring that the narratives and visual elements are seamlessly interconnected.
% accompany spatiotemporal data visualizations for better understanding, which necessitates appropriate integration during video playback.

% Research~\cite{chen2021changing} indicates that narratives from a first-person perspective foster a more immersive and connected experience, while those from a third-person viewpoint offer a broader reflection on character interactions and their implications. 

% To achieve comprehensive narration generation for sports tactics, 
% we require a powerful LLM that can not only infer the current situation of actions but also deduce the causal relationship between multiple actions. 

\para{R2. Explaining Tactics with Grounded Video Data.} %% based on the data extracted from video, hullicination 
A fundamental aspect of our approach involves ensuring that the explanations generated are grounded in the actual video, avoiding any form of ``hallucination'' of LLMs~\cite{}. 
This consideration is crucial for maintaining the reliability of the tactical explanation provided by \ourtool{}.
By anchoring our explanations in the tactics and observable actions within the video,
we can offer users insights that are not only accurate but also verifiable against the source material. 
This requires a understanding of the video.
Specifically, we need to detect the tactic itself, as well as all the actions that potentially involved.


% require a storytelling approach that allows for the effective and intuitive presentation of information through visualization, 
\para{R3. Explaining Tactics using Embedded Visualizations.} %% 3 Action Vis + dialouge bubble
To enrich the explanation of tactics, it is essential to complement the narratives with visual representations, creating an experience akin to watching a film~\cite{gershon2001storytelling}. 
This requires the careful design of embedded visualizations for the key actions within the narratives. 
Each action demands specific animated embedded visualizations
to capture its unique objectives and to dynamic nature.
Furthermore, the visual explanation must also reflect the chosen narrative perspective.
% bridging the narrative to the visual elements effectively. 
For instance, in a first-person narrative, 
the narration should directly connect to specific subjects within the visualization. 
In contrast, a third-person narrative allows for a more generalized correlation between the visualizations and the narration.
The overarching challenge for \ourtool{} is to seamlessly integrate these visual explanations within the video content, ensuring a cohesive and engaging presentation of tactical explanation. 


% In order to better explain the tatics,
% we further require to visually present the generated narrative explainastion, 
% akin to the experience of watching a film~\cite{gershon2001storytelling}. 
% To this end, we need to design intuitive \emph{embedded visualizations} for the key actions,
% Each action has their own considerations and objectives, and should be animated
%  to relfect the dyanmic process.
% Moreover, we should also visually reflect the narrative perspectives of the explaination.
% For instance, in a first-person narrative, the narration should directly connect to specific subjects within the visualization. 
% In contrast, a third-person narrative allows for a more generalized correlation between the visualizations and the narration.
% All together, the challenge for \ourtool{} lies in seamlessly visualize the explainations together with the video. 

% Building upon the narrative approach to explaining tactics, we recognize the importance of complementing these narratives with embedded visualizations, much like the enriched experience offered by film storytelling (Gershon, 2001). To elevate our users' understanding of tactics, it's crucial to present the narratively explained tactics through intuitive visual representations. These embedded visualizations are designed to vividly depict key actions, mirroring the dynamic nature of the game through animation. Each action visualization is crafted with specific considerations and objectives in mind, ensuring that the essence of each strategic move is captured accurately and engagingly.

% Furthermore, these visualizations need to reflect the narrative perspective employed in the explanation. For example, when using a first-person narrative, the visualization should create a direct link between the narration and specific subjects within the scene, immersing the viewer in the personal experience of the player described. Conversely, a third-person narrative perspective benefits from a broader, more omniscient correlation between the visuals and the narration, offering viewers a comprehensive overview of the tactics in play.

% The challenge for \ourtool{} lies in the seamless integration of these visual explanations with the ongoing video content. This requires a delicate balance between narrative clarity, visual intuitiveness, and the dynamic flow of the game, ensuring that the tactical insights are both accessible and captivating for the viewer. Through this innovative approach, we aim to not only inform but also deeply engage our audience in the tactical intricacies of the game.


% Meanwhile, each technique encompasses different visualization and narration design considerations. 
% For the first-person perspective, narration needs to be tied to specific subjects in the visualization, 
% while in the third person, the connection between visualizations and narration can be more subtle. 
% integrating various storytelling techniques with corresponding visualizations that align with the selected narrative approach. 


% Thus, it's essential for \ourtool{} to accommodate various storytelling techniques and incorporate appropriate visualizations to match the chosen narrative method.


% Furthermore, \textbf{animations} are essential for visually distinguishing among the complex movements, highlighting key players and actions. 
% Therefore, a second design goal of \ourtool{} is to answer tactics and in-game decisions with the automatic creation of narration, embedded visualization, and animations.

%% Embedded visualizations
% \textbf{embedded visualizations} are required to highlight critical actions, i.g., the pass, the screen, and the cut within the game video. 
% For each action, specific considerations are necessary. 
% For a pass, it is essential to clearly indicate the players giving and receiving the pass. 
% In the case of a screen, one player must obstruct another player's movement, 
% and for a cut, the objective is to evade the defense and move into a broader offensive position. 
% Visualization designs are required to depict these actions clearly. 





%%%%%%
% To describe the details for tactics, \ourtool{} needs to consider three key components, including \textbf{narration} of action sequences to explain the logic, 
% \textbf{embedded visualization} to specify individual actions, 
% and \textbf{animations} to highlight main movement. 

\subsection{System Overview}
Based on the considerations, we design \ourtool{}, a VQA system with three major components, namely,
a Narrative Agent (\autoref{fig:system}b),
a data processor (\autoref{fig:system}a),
and a visualizer (\autoref{fig:system}c).
The core of \ourtool{} is a LLM-based agent, so called Narrative Agent.
It takes the user's question as the input and the data extract from the video as the context
to generate an explanation,
which is then visualized using embedded visualization.
In the following sections, we will introduce the detail of each component.

% Based on the design requirements analyzed in Section 3, we introduce \ourtool{}, a visual question-answering (VQA) system designed to elucidate complex questions (R1), such as those related to strategy and in-game decisions (R2). This tool combines narrative and visualization techniques for effective storytelling (R3). \ourtool{} consists of two pipeline parts that allow users to ask not only strategic and in-game decision questions but also performance- and stats-based questions.

==> sections/backup/4LLMAgent_v2.tex <==
\section{Narrative Agent}
\label{sec:llm_core}

To facilitate the understanding of the tactic (R2),
we aim to generate the explanation in a form of narratives (i.e., story).
We achieve this through \emph{prompt engineering}.
This section introduce how we design the prompt.


For tactic-related questions, 
we employ the RAG framework, which supplements LLMs with external knowledge. 
This is especially useful for domain-specific questions, allowing the LLM to leverage a wide range of external knowledge without the need to be retrained for task-specific applications. 
RAG's effectiveness in enhancing conversational agents~\cite{lewis2020retrieval, gao2023retrieval} illustrates its potential in applications like ours.
The template above shows our prompt for tactic-based questions. 
Our RAG prompting technique includes three key components:


% \subsection{Answering Tactic-based Questions with RAG}
% The LLM achieve human-level performance across a wide range of tasks (e.g., professional benchmarks)~\cite{achiam2023gpt}, demonstrating its capabilities to comprehend the complex contexts of in-game decisions and generate reasonable answers to basketball strategic questions. (In our implementatoin, we used a OpenAI API with gpt-4-0125-preview model.) To produce storytelling-based strategic answer, the LLM is utilized to create narratives based on the user's question, a series of actions, tactical information, and prompts, as shown in \autoref{fig:system} (B-1). To be specific, the prompts play a crucial role in a consistent narrative and answer format to link visualization.



\para{Providing Additional Context.}
We enrich the the user's input with additional game context of the current video clip,
including \texttt{Player Information}, detected \texttt{Tactics}, and \texttt{Actions}.
This information is extracted from the video clip by using external machine learning models (which will be detailed in Sec.~\ref{}),
and provided as structural text.
For each query, the system dynamically loads game context relevant to the video clip, 
enabling the LLM to tailor its responses to the specific clip in question.
Details on the structural format can be found in the supplementary materials.

\para{Generating Explanations with Narratives.}
\zt{should talk about how we generate explainations with narratives, two steps}
To enhance the comprehension of explanations, we adopt a top-down approach—presenting a strategic overview before delving into detailed actions. 
Our pilot experiments indicated that LLMs often struggle with generating comprehensive explanations in a single attempt. 
To address this, we've divided the task into two distinct steps, in line with established best practices~\cite{shen2023data}. 
Initially, we prompt the LLM to produce an overview explanation of the tactics.
This overview succinctly summarizes the tactics, enabling fans to grasp the essentials of tactical unfolding.
Subsequently, 
we prompt the LLM to generate a detailed, sequential breakdown of the tactics,
providing users with step-by-step insights into specific actions and decision-making processes. 
This two-step approach not only refines the LLM’s output by incorporating detailed constraints but also safeguards against the generation of incorrect explanatory formats.

\para{Formatting Explanations with Various Perspectives.}
To address R3, 
we apply additional constraints to structure format of the generated explanations,
facilitating their mapping to visualizations (Sec.~\ref{}).
Moreover, to generate explanations from a first-person perspective, an approach not typically produced by LLMs, 
we add prompts that guide the model to produce responses 
(e.g., \textit{... answer should be a format of a conversation or a role-play dialogue between two players...}),
including descriptions that evoke a first-person reaction to in-game actions (e.g., \textit{... screen elicit a surprised or shocked reaction from the other person...}).
An example format is provided to ensure answer consistency, given the challenge of maintaining uniform response formats due to the varied nature of actions and tactics. 




% We include additional descriptions for the first person perspective () and describe the how the model react in the action as first person perspective (\textit{... screen elicit a surprised or shocked reaction from the other person ... }). 
% We provide an example of answer format to ensure consistency, as the keeping the same answer format is challenging for the LLM due to diverse actions and tactics. 
% The outputs of LLM are utilized for generating strategic and in-game decision answer, as shown in \autoref{fig:system} (C). 
 % data for the relevant video clip, enabling users to pose strategic questions about any moment in the game.
 % The inclusion of this detailed context, fully described in the supplementary materials, is designed to inform the model's responses more effectively. 
 
% Instead of providing LLM only the user's question,
% we further provide extra information of the game as the context,
% and ask LLM to generate the responde based on the context information.
% Specifically, in our prompt template, we provide the \texttt{Player information}, the detected \texttt{Tactic},
% and the detected \texttt{Actions} of the current video clip.
% This information is all provided as structured text, with details are provided in the supplymental materials.
% We load all needed data for each individual clip for the users' request, allowing users to ask strategic question every clip.

% Subsequently, we provide various structure of prompts like \autoref{fig:system} (B-1) (e.g., constrains, player information, answer format, and actions), which elucidate the reasons why offensive players perform specific actions such as \textit{disturb the defense}, \textit{overcome tight defense}, \textit{create space for other players}, and etc. This information helps LLM interpret the logic behind the players' movement and understand the in-game decisions among players. We define the answer format by separating each action with a delimiter, gaining a third person perspective answers.







% \ourtool{} not only explain tactical question but also support basic players' information, metadata (e.g., ranking, historical performance of team), performance, and stats-based question.
% To answer basic information of both players and teams, we leverage a ReAct \cite{yao2022react}.
% ReAct performs acting and reasoning based on the LLM, allowing LLM to mimic human-like task-solving.
% For example, when a user ask about Stephen Curry's shooting percentage, this system will interact with tools (e.g., wikipedia search) and do reasoning for the responses from tools. By doing this repetitively, the LLM can find reasonable answers for the questions.
% We provide multiple actioning tools for the LLM to obtain information within the game (e.g., Python and pandas)
% or outsie the game (e.g., Google Search api, Wikipedia search api and Statmuse api)



% LangChain~\cite{Langchain}, a framework for developing LLM applications, to retrieve different sources of context that we provide and to do reasoning based on the given context. We define several tools for providing context to the LLM, including  \cite{Statmuse24}, as shown in \autoref{fig:system} (B-2). 

% \textbf{Retrieving stats data in the game} 
% The fans also inquire about the current game such as \textit{the number of fouls in this game?}. To answer this, we utilize the ReAct\cite{yao2022react} with Python and pandas tools to retrieve statistics of the game from stats data \autoref{fig:system} (B-2). All the response will be the output of performance and stats based questions.


==> sections/backup/4system_v1.tex <==

\section{System}
Based on the design requirements analyzed in Section 3, we introduce \ourtool{}, a visual question-answering (VQA) system designed to elucidate complex questions (R1), such as those related to strategy and in-game decisions (R2). This tool combines narrative and visualization techniques for effective storytelling (R3). \ourtool{} consists of two pipeline parts that allow users to ask not only strategic and in-game decision questions but also performance- and stats-based questions.

\subsection{Answering strategic and in-game questions}
As shown in \autoref{fig:system}, answering strategic and in-game questions involves a complex process. This process includes extracting the positions and bounding boxes of ball and players (\autoref{fig:system} A-1), detecting actions from the data (\autoref{fig:system} A-2), classifying tactics (\autoref{fig:system} A-3), and generating reasonable outputs from large language model (LLM) (\autoref{fig:system} B-1). \ourtool{} generates the embedded visualization (\autoref{fig:system} (B-3)) based on data from \autoref{fig:system} (A-1 and 2). One important aspect is to convert the spatial information to LLM's input. We decide to use LLM with textual information rather than multi-modal LLM which can take images or videos. The performance of current multi-modal LLM is not sufficient to explain strategies and in-game decisions in the sports. Our solution is to pre-process all data that need to produce the explanation by using computer vision pipeline and make those data to textual information that easily adopt to current LLM. To do this, we utilize prior research \cite{chen2023iball} that includes datasets tracking the bounding boxes of both the ball and players. The dataset has the bounding boxes ball and players every frame. The ball owner is calculated by the closest player with ball. We utilize x and y position in court from the SportVU \cite{SportVU24} to classify tactics and recognize which player is in one-on-one relationship or defending to detect the actions.



\subsubsection{Action Detection}
\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{figs/action_graph.png}
\caption{An action list displays the series of actions performed by offensive players, including Pass, Cut, Screen, and Shoot. The main actions are identified based on ball movement or movements that enhance scoring opportunities, such as Shoot or Pass the ball. To extract the main actions related to Pass and Shoot, we establish criteria to filter out the less significant actions between Cuts and Screens.}
\label{fig:action_graph}
\end{figure}

Detecting actions from players' movements in the video plays an important role in explaining strategies and in-game decisions and satisfying the requirement (R2). A strategy consists of a series of actions, which are players' movements, such as a screen, a pass, and a cut \cite{sicilia2019deephoops}. As shown in \autoref{fig:system} (A-2), we define four different actions: the screen, the pass, the cut, and the shoot, as follows:
\begin{itemize}
    \item \textbf{Screen}: Player A attempts to block or delay a defender to create space and time for moving to a better position for offense or a shot \cite{tian2019use}. More technically, an offensive player performs a screen on a defender who is marking another offensive player with the ball at a close distance. We compute the \textit{distances} among players to check offensive players are close to defensive players and identify offensive players who change their one-on-one relationship.
    \item \textbf{Pass}: Player A sends the ball to his teammate B, who has a higher chance of scoring at the basket. We detect the pass by observing changes in the \textit{ball owner} within the same team, checking every frame.
    \item \textbf{Cut}: A cut is performed by a player without possession of the ball. The player moves from one location to another on the court to create space or move away from a defender, aiming for better offensive opportunities \cite{courel2018inside, tian2019use}. Since it is easier for a defender to guard a stationary offensive player, the offensive player moves quickly to another region to evade defense. We divide the court into 10 sub-regions, such as key, post, wing, etc., \cite{unkown10glossary}, and detect offensive players who move at 6 feet per second speed \cite{Wu2022OBTrackerVA} to a different area.    
    \item \textbf{Shoot}: A shot marks the end of an offense, and possession will change whether the player makes or misses the points. We detect changes in ball possessions between the two teams.
\end{itemize}

Another important aspect is the extraction of significant actions, since many different actions will be captured by our above criteria.
The redundant ones that are not crucial to strategies lead to degrade the user experience to show all actions. One solution is to choose important actions. The pass is the most significant factors to deploy strategies, and shooting is an essential part of scoring points in basketball \cite{tian2019use}. As shown in \autoref{fig:action_graph}, we identify the main actions as pass and shoot, while the other actions such as cut and screen can be sub actions, since some irrelevant or less important cuts and screens disrupt the explanation of the strategy. We build an action list to filter out irrelevant actions. We filter out that the cuts do not directly affect receiving a pass, while the screens do not aid players who have the ball or will receive the ball based on distance between the players and screen position. For example, one player cannot receive the ball from the cut in \autoref{fig:action_graph} (1), then the cut is disconnected. Similarly, the screen in \autoref{fig:action_graph} (2) is performed but does not have a huge impact to proceed play and disconnected and excluded based on distance between screen position and previous and next passes. The outputs of action detection are action type with frame index and the coordinates of players.

% in game decision

\subsubsection{Tactic Detection}
To classify tactics, we take players' coordinate data (e.g,. x and y position on the court) from SportVU \cite{SportVU24} and predict the label of tactics, as shown in \autoref{fig:system} (A-3).
To build a classifier model, we utilize data for the movement of players that match with specific tactics \cite{tsai2017recognizing}. The data includes x and y coordinates of each individual player on the courts as normalized values, along with the tactic label such as Back-Side Pick and Roll, Elevator, Pin-Down, etc. It consist of only 134 tactics in total, making it challenging to apply deep learning or complex models. A K-Nearest Neighbors (KNN) algorithm is a reasonable solution \cite{tian2019use} since it is able to identify a K number of similar data points based on its distance metrics (e.g., Euclidean distance.) We trained this algorithm using the existing tactic data \cite{tsai2017recognizing} to predict tactic label for the new input data. Another important aspect is that we use fastDTW \cite{salvador2007toward}, a refined version of Dynamic Time Warping (DTW) that is optimized linear and time and space complexity. The DTW is a method used to calculate the similarity between two time series, allowing one of the series to be non-linearly adjusted by expanding or compressing its timeline. This adjustment is crucial to match the difference lengths clips for computing the similarity between data, since the duration of clips vary. After classifying tactic, the information tactic will be provided to LLM.

\subsubsection{Storytelling and different narrative perspective}
To generate strategic answers and diverse narrative perspectives, we leverage the ability of a large language model (LLM) to satisfy design requirement (R2). The LLM achieve human-level performance across a wide range of tasks (e.g., professional benchmarks) \cite{achiam2023gpt}, demonstrating its capabilities to comprehend the complex contexts of in-game decisions and generate reasonable answers to basketball strategic questions. (In our implementatoin, we used a OpenAI API with gpt-4-0125-preview model.) To produce storytelling-based strategic answer, the LLM is utilized to create narratives based on the user's question, a series of actions, tactical information, and prompts, as shown in \autoref{fig:system} (B-1). To be specific, the prompts play a crucial role in a consistent narrative and answer format to link visualization.

Answering the strategic and in-game decisions is two main components: a brief summary of tactics and an explanation that incorporates a serious actions and visualization. Initially, \ourtool{} provides a brief summary of tactic to allows the fans to understand the concise descriptions of tactics and how to unfold the tactics, using LLM based on tactic descriptions and actions. After the summary, the users can watch the video clip with action visualization and narratives. This two-step process enhances the LLM's performance by including detailed information and preventing incorrect answer formats. Subsequently, we provide various structure of prompts like \autoref{fig:system} (B-1) (e.g., constrains, player information, answer format, and actions), which elucidate the reasons why offensive players perform specific actions such as \textit{disturb the defense}, \textit{overcome tight defense}, \textit{create space for other players}, and etc. This information helps LLM interpret the logic behind the players' movement and understand the in-game decisions among players. We define the answer format by separating each action with a delimiter, gaining a third person perspective answers.

To meet the requirement (R3), we modify the prompts related constraints to produce a first person perspective that is not common response type for the LLM. We include additional descriptions for the first person perspective (\textit{... answer should be a format of a conversation or a role-play dialogue between two players ...}) and describe the how the model react in the action as first person perspective (\textit{... screen elicit a surprised or shocked reaction from the other person ... }). We provide an example of answer format to ensure consistency, as the keeping the same answer format is challenging for the LLM due to diverse actions and tactics. The outputs of LLM are utilized for generating strategic and in-game decision answer, as shown in \autoref{fig:system} (C). We load all needed data for each individual clip for the users' request, allowing users to ask strategic question every clip.


\subsection{Answering performance and stats based questions}
Recent studies \cite{lin2022quest, chen2023iball} shows that the casual fans are interested in knowing stats information as mentioned in Sec. 3. \ourtool{} not only explain strategic question but also support basic players' information, metadata (e.g., ranking, historical performance of team), performance, and stats-based question.
\textbf{Searching basic information.}
To answer basic information of both players and teams, we leverage LangChain \cite{Langchain}, a framework for developing LLM applications, to retrieve different sources of context that we provide and to do reasoning based on the given context. We define several tools for providing context to the LLM, including Google Search api, Wikipedia search api and Statmuse api \cite{Statmuse24}, as shown in \autoref{fig:system} (B-2). The framework, ReAct \cite{yao2022react}, performs acting and reasoning based on the LLM, allowing LLM to mimic human-like task-solving. For example, when a user ask about Stephen Curry's shooting percentage, this system will interact with tools (e.g., wikipedia search) and do reasoning for the responses from tools. By doing this repetitively, the LLM can find reasonable answers for the questions.
\textbf{Retrieving stats data in the game} 
The fans also inquire about the current game such as \textit{the number of fouls in this game?}. To answer this, we utilize the ReAct\cite{yao2022react} with Python and pandas tools to retrieve statistics of the game from stats data \autoref{fig:system} (B-2). All the response will be the output of performance and stats based questions.



%although important for the successful execution of a team’s game plan, are rarely evaluated. Even when we have volume
%statistics from these actions, the context is usually absent, which makes it hard to evaluate the importance of each of these
%actions. For example, simply counting passes can be very misleading; a pass exchange in the backcourt is certainly not as valuable as a pass that leads to an open three point shot.



==> sections/backup/4system_v2.tex <==
\section{Narrative Agent}
\label{sec:llm_core}

To fulfill R1, our system should be able to 1) accurately interpret users' natural language queries, and 2) generate insightful explanations in response.
Leveraging LLM provides a promising solution to accomplish these objectives.
However, generating meaningful explanations requires the LLM to comprehend the content within a basketball video.
Although multi-modal LLMs are capable of processing image data,
they often underperform in domain-specific tasks~\cite{},
such as detecting actions or tactics from a sports video. 
To overcome this challenge, our methodology employs a text-only LLM, which is enhanced by integrating a Retrieval-Augmented Generation (RAG) framework~\cite{lewis2020retrieval} 
and a Reasoning-and-Actioning (ReAct) prompting strategy~\cite{yao2022react}
for different types of questions.
 
\subsection{Answering Tactic-based Questions with RAG}
% The LLM achieve human-level performance across a wide range of tasks (e.g., professional benchmarks)~\cite{achiam2023gpt}, demonstrating its capabilities to comprehend the complex contexts of in-game decisions and generate reasonable answers to basketball strategic questions. (In our implementatoin, we used a OpenAI API with gpt-4-0125-preview model.) To produce storytelling-based strategic answer, the LLM is utilized to create narratives based on the user's question, a series of actions, tactical information, and prompts, as shown in \autoref{fig:system} (B-1). To be specific, the prompts play a crucial role in a consistent narrative and answer format to link visualization.

\begin{coloredquotation}
    \textbf{Prompt template:}\\
    Please explain question \{ user question \} based on the following context:
    \begin{itemize}
        \item \{ \texttt{Player Information} \}
        \item \{ \texttt{Detected Tactics} \}
        \item \{ \texttt{Detected Actions} \}
    \end{itemize}
    
    Your explanation should follow the below constraints and formats:
    \begin{itemize}
        \item \{ \texttt{Constraints} \}
        \item \{ \texttt{Format} \}
    \end{itemize}
\end{coloredquotation}

\noindent
For tactic-related questions, 
we employ the RAG framework, which supplements LLMs with external knowledge. 
This is especially useful for domain-specific questions, allowing the LLM to leverage a wide range of external knowledge without the need to be retrained for task-specific applications. 
RAG's effectiveness in enhancing conversational agents~\cite{lewis2020retrieval, gao2023retrieval} illustrates its potential in applications like ours.
The template above shows our prompt for tactic-based questions. 
Our RAG prompting technique includes three key components:

\para{Providing Additional Context.}
We enrich the the user's input with additional game context of the current video clip,
including \texttt{Player Information}, detected \texttt{Tactics}, and \texttt{Actions}.
This information is extracted from the video clip by using external machine learning models (which will be detailed in Sec.~\ref{}),
and provided as structural text.
For each query, the system dynamically loads game context relevant to the video clip, 
enabling the LLM to tailor its responses to the specific clip in question.
Details on the structural format can be found in the supplementary materials.

\para{Formatting Explanations with Various Perspectives.}
To address R3, 
we apply additional constraints to structure format of the generated explanations,
facilitating their mapping to visualizations (Sec.~\ref{}).
Moreover, to generate explanations from a first-person perspective, an approach not typically produced by LLMs, 
we add prompts that guide the model to produce responses 
(e.g., \textit{... answer should be a format of a conversation or a role-play dialogue between two players...}),
including descriptions that evoke a first-person reaction to in-game actions (e.g., \textit{... screen elicit a surprised or shocked reaction from the other person...}).
An example format is provided to ensure answer consistency, given the challenge of maintaining uniform response formats due to the varied nature of actions and tactics. 

\para{Generating Explanations in Two Steps.}
To enhance the comprehension of explanations, we adopt a top-down approach—presenting a strategic overview before delving into detailed actions. 
Our pilot experiments indicated that LLMs often struggle with generating comprehensive explanations in a single attempt. 
To address this, we've divided the task into two distinct steps, in line with established best practices~\cite{shen2023data}. 
Initially, we prompt the LLM to produce an overview explanation of the tactics.
This overview succinctly summarizes the tactics, enabling fans to grasp the essentials of tactical unfolding.
Subsequently, 
we prompt the LLM to generate a detailed, sequential breakdown of the tactics,
providing users with step-by-step insights into specific actions and decision-making processes. 
This two-step approach not only refines the LLM’s output by incorporating detailed constraints but also safeguards against the generation of incorrect explanatory formats.

% We include additional descriptions for the first person perspective () and describe the how the model react in the action as first person perspective (\textit{... screen elicit a surprised or shocked reaction from the other person ... }). 
% We provide an example of answer format to ensure consistency, as the keeping the same answer format is challenging for the LLM due to diverse actions and tactics. 
% The outputs of LLM are utilized for generating strategic and in-game decision answer, as shown in \autoref{fig:system} (C). 
 % data for the relevant video clip, enabling users to pose strategic questions about any moment in the game.
 % The inclusion of this detailed context, fully described in the supplementary materials, is designed to inform the model's responses more effectively. 
 
% Instead of providing LLM only the user's question,
% we further provide extra information of the game as the context,
% and ask LLM to generate the responde based on the context information.
% Specifically, in our prompt template, we provide the \texttt{Player information}, the detected \texttt{Tactic},
% and the detected \texttt{Actions} of the current video clip.
% This information is all provided as structured text, with details are provided in the supplymental materials.
% We load all needed data for each individual clip for the users' request, allowing users to ask strategic question every clip.

% Subsequently, we provide various structure of prompts like \autoref{fig:system} (B-1) (e.g., constrains, player information, answer format, and actions), which elucidate the reasons why offensive players perform specific actions such as \textit{disturb the defense}, \textit{overcome tight defense}, \textit{create space for other players}, and etc. This information helps LLM interpret the logic behind the players' movement and understand the in-game decisions among players. We define the answer format by separating each action with a delimiter, gaining a third person perspective answers.






\subsection{Answering Stats-based Questions with ReAct}
\ourtool{} also supports statistics-based questions, such as inquiries related to basic player information, team rankings, and historical performance.
We utilize a framework named ReAct~\cite{yao2022react}, which enhances LLMs by enabling them to perform tasks and reason in a manner akin to human problem-solving. 
For instance, if a user inquires about Stephen Curry's shooting percentage, the system employs ReAct to interact with various tools, such as Wikipedia searches, engaging in a process of querying and reasoning based on the responses from these tools. 
Through this iterative process, the LLM is able to derive well-founded answers.
We equip \ourtool{} with multiple tools for retrieving information within and outside the game context.
These include programming tools like Pandas for in-game data analysis, as well as external APIs for web searches, including Google Search API, Wikipedia search API, and Statmuse API for broader information gathering.

% \ourtool{} not only explain tactical question but also support basic players' information, metadata (e.g., ranking, historical performance of team), performance, and stats-based question.
% To answer basic information of both players and teams, we leverage a ReAct \cite{yao2022react}.
% ReAct performs acting and reasoning based on the LLM, allowing LLM to mimic human-like task-solving.
% For example, when a user ask about Stephen Curry's shooting percentage, this system will interact with tools (e.g., wikipedia search) and do reasoning for the responses from tools. By doing this repetitively, the LLM can find reasonable answers for the questions.
% We provide multiple actioning tools for the LLM to obtain information within the game (e.g., Python and pandas)
% or outsie the game (e.g., Google Search api, Wikipedia search api and Statmuse api)



% LangChain~\cite{Langchain}, a framework for developing LLM applications, to retrieve different sources of context that we provide and to do reasoning based on the given context. We define several tools for providing context to the LLM, including  \cite{Statmuse24}, as shown in \autoref{fig:system} (B-2). 

% \textbf{Retrieving stats data in the game} 
% The fans also inquire about the current game such as \textit{the number of fouls in this game?}. To answer this, we utilize the ReAct\cite{yao2022react} with Python and pandas tools to retrieve statistics of the game from stats data \autoref{fig:system} (B-2). All the response will be the output of performance and stats based questions.


==> sections/backup/5data_processing_v1.tex <==

\section{Data Processor}

To generate reliable explations (R1),
we should extract data from the video clip in question to provide a context for the LLM.
This section details how we detect the current tactics and involved actions. 
We tackle them separately by using a combination of machine learning methods.

% Figure 2 illustrates the complexity of answering tactics and in-game questions. 
% Based on R1, we should extract data from 

% how tactic-based questions require external knowledge from the video clip, including detecting 

% As shown in \autoref{fig:system}, answering tactics and in-game questions involves a complex process. 
% As explained in Sec.~\ref{sec:llm_core}, answering tactic-based questions involves external knowledge extracted from the video clip in question. 


% This process includes extracting the positions and bounding boxes of ball and players (\autoref{fig:system} A-1), detecting actions from the data (\autoref{fig:system} A-2), classifying tactics (\autoref{fig:system} A-3)
% , and generating reasonable outputs from large language model (LLM) (\autoref{fig:system} B-1). \ourtool{} generates the embedded visualization (\autoref{fig:system} (B-3)) based on data from \autoref{fig:system} (A-1 and 2). 

\subsection{Tactic Detection}
\label{sec:tactic}
Identifying the tactics used by teams is crucial for answering tactic-based questions.
Our approach to tactic detection relies on the classification of team tactics by analyzing 
the movement patterns of the five offensive players on the court.
These patterns are represented by the five temporal sequence of their coordinates,
each denoted as $\{(x, y)\}_{i=0}^t$, with $x$ and $y$ are the on-court position, and $t$ marking the clip's end frame. 
Specifically, we leverage the K-Nearest Neighbors (KNN) algorithm and a reference dataset that includes 134 annotated clips. Each annotated clip contains the temporal sequences of the five offensive players' coordinates,
and the associated offensive tactic, such as Back-Side Pick and Roll, Elevator, or Pin-Down. 
We classify the tactic of the current video clip by comparing movement patterns to those in a reference dataset, identifying the tactic type that best matches a clip in the dataset.

Given the difference in sequence length between video clips,
it is impractical to use the traditional Euclidean distance for the KNN algorithm's distance metric. 
Consequently, we adopt FastDTW, a refined variant of Dynamic Time Warping (DTW), to overcome this challenge. 
FastDTW~\cite{salvador2007toward} can calculate the similarity distance between two temporal sequences of different lengths, 
thus offering a robust solution for our need.
\zt{accuracy?}

% from SportVU \cite{SportVU24} and predict the label of tactics, as shown in \autoref{fig:system} (A-3).
% Our solution is to pre-process all data that need to produce the explanation by using computer vision pipeline and make those data to textual information that easily adopt to current LLM. 
% To do this, we utilize prior research~\cite{chen2023iball} that includes datasets tracking the bounding boxes of both the ball and players. The dataset has the bounding boxes ball and players every frame. The ball owner is calculated by the closest player with ball. We utilize x and y position in court from the SportVU \cite{SportVU24} to classify tactics and recognize which player is in one-on-one relationship or defending to detect the actions.

\subsection{Action Detection and Filtering}
\label{sec:action}
\begin{figure}[h]
\centering
\includegraphics[width=\columnwidth]{figs/action_graph.png}
\caption{An action list displays the series of actions performed by offensive players, including Pass, Cut, Screen, and Shoot. The primary actions are identified based on ball movement or movements that enhance scoring opportunities, such as Shoot or Pass the ball. To extract the primary actions related to Pass and Shoot, we set criteria to filter out secondary actions like Cuts and Screens, identified by actions 1 and 2 in red circles.}
\label{fig:action_graph}
\end{figure}

\noindent
Detecting actions from players' movements in the video plays an important role in explaining tactics and satisfying the requirement (R1). 
According to previous work~\cite{sicilia2019deephoops}, a tactic consists of a series of actions.
In this work, we focus on four most important actions in a basketball offensive tactic:
\begin{itemize}
    
    
    % compute \emph{distances} to check offensive players are close to defensive players 
    % and identify offensive players who change their one-on-one relationship.
    % This analysis helps us detect instances where offensive players come into close proximity with defenders and alter their direct defensive assignments.
       
    % This analysis helps us detect instances where offensive players    
    % means if a player attempts to block or delay a defender to create space and time for moving to a better position for offense or a shot. 
    % More technically, an offensive player performs a screen on a defender who is marking another offensive player with the ball at a close distance. 
    % with a frame-by-frame analysis ensuring accurate detection.
    % Player A sends the ball to his teammate B, who has a higher chance of scoring at the basket. We detect the pass by observing changes in the \textit{ball owner} within the same team, checking every frame.
    \item \Shoot{} results in a change of possession regardless of whether it scores. 
    We detect a Shot action if the ball possession changes between the two teams.

    \item \Pass{} occurs when a player transfers the ball to a teammate, who is in a more advantageous position to score. A pass is identified by tracking \emph{ball ownership} changes  within the same team.
    
    \item \Cut{} is performed by a player who doesn't have the ball.
    The player moves swiftly from one court area to another to either create space or distance from a defender, thus enhancing offensive possibilities~\cite{courel2018inside, tian2019use}. 
    This cut action is particularly effective against defenders as stationary players are easy to be guard.
    For detection, we segment the court into 10 sub-regions (e.g., key, post, wing), following a  taxonomy~\cite{unkown10glossary}.
    Then, a Cut action is detected if an offensive players moves at a speed of 6 feet per second or faster to a different sub-region~\cite{Wu2022OBTrackerVA}.

    \item \Screen{} refers to an offensive player's attempt to block or slow down a defender, thereby creating space and time for a teammate to move into a more advantageous offensive position or to take a shot~\cite{tian2019use}.
    From a technical standpoint, a screen occurs when an offensive player blocks a defender who is closely guarding another offensive player with possession of the ball. 
    To identify when a screen is being set, we analyze the \emph{distances} between players on the court. 
    A Screen action is detected if an offensive player changes their marking or covering player.
    

\end{itemize}

After detecting the actions in the video clips,
we still need to identify the \emph{important} ones.
Not all captured actions are relevant to the tactic framework of a game; including redundant or non-crucial actions could diminish the user experience by cluttering the presentation with unnecessary details. 
A practical approach to streamline this process is to prioritize key actions integral to tatic implementation and scoring. 
According to Tian et al.~\cite{tian2019use}, 
Pass plays a pivotal role in executing strategies, 
while Shoot is fundamental to scoring points. 
As illustrated in \autoref{fig:action_graph}, 
we categorize Pass and Shoot as primary actions, 
considering Cut and Screen as secondary actions. 
This distinction helps in filtering out irrelevant or less impactful actions that do not contribute meaningfully to the tactic explanation.

Then, we filter out the ineffective secondary actions,
including 1) cuts that are not followed by to a ball receive
and 2) screens that are not positioned to benefit the ball handler or the intended receiver, based on the proximity of players and the location of the screen.
% For instance, a cut depicted in Figure X (1) that fails to position a player to receive the ball is deemed irrelevant and excluded. Similarly, a screen shown in Figure X (2) that does not significantly influence the play's progression, due to the distance between the screen set and the trajectory of preceding and subsequent passes, is also filtered out.
For example, one player cannot receive the ball after the cut in \autoref{fig:action_graph} (1), then the cut is disconnected. Similarly, the screen depicted in \autoref{fig:action_graph} (2) is performed but does not have a huge impact to proceed play and disconnected and excluded based on distance between screen position and previous and next passes. The outputs of action detection are action type with frame index and the coordinates of players.
The result of this selective process is a list of actions, each associated with its type, frame index, and the coordinates of the involved players, ensuring a focused and meaningful analysis of game tactics.

\subsection{Answering Stats-based Questions with ReAct}
\ourtool{} also supports statistics-based questions, such as inquiries related to basic player information, team rankings, and historical performance.
We utilize a framework named ReAct~\cite{yao2022react}, which enhances LLMs by enabling them to perform tasks and reason in a manner akin to human problem-solving. 
For instance, if a user inquires about Stephen Curry's shooting percentage, the system employs ReAct to interact with various tools, such as Wikipedia searches, engaging in a process of querying and reasoning based on the responses from these tools. 
Through this iterative process, the LLM is able to derive well-founded answers.
We equip \ourtool{} with multiple tools for retrieving information within and outside the game context.
These include programming tools like Pandas for in-game data analysis, as well as external APIs for web searches, including Google Search API, Wikipedia search API, and Statmuse API for broader information gathering.

% following these rules:
% - 
% directly contribute to receiving a pass
% cuts do not directly affect receiving a pass, 
% - 
% screens do not aid players who have the ball or will receive the ball based on distance between the players and screen position

% Another important aspect is the extraction of significant actions, 
% since many different actions will be captured by our above criteria.
% The redundant ones that are not crucial to strategies lead to degrade the user experience to show all actions. 
% One solution is to choose important actions. 

% The pass is the most significant factors to deploy strategies, and shooting is an essential part of scoring points in basketball \cite{tian2019use}. 
% As shown in \autoref{fig:action_graph}, we identify the main actions as pass and shoot, while the other actions such as cut and screen can be sub actions,
% since some irrelevant or less important cuts and screens disrupt the explanation of the strategy. 





%although important for the successful execution of a team’s game plan, are rarely evaluated. Even when we have volume
%statistics from these actions, the context is usually absent, which makes it hard to evaluate the importance of each of these
%actions. For example, simply counting passes can be very misleading; a pass exchange in the backcourt is certainly not as valuable as a pass that leads to an open three point shot.



==> sections/backup/5system_v2.tex <==

\section{System}
Based on the design requirements analyzed in Section 3, we introduce \ourtool{}, a visual question-answering (VQA) system designed to elucidate complex questions (R1), such as those related to strategy and in-game decisions (R2). This tool combines narrative and visualization techniques for effective storytelling (R3). \ourtool{} consists of two pipeline parts that allow users to ask not only strategic and in-game decision questions but also performance- and stats-based questions.

\subsection{Answering strategic and in-game questions}
As shown in \autoref{fig:system}, answering strategic and in-game questions involves a complex process. This process includes extracting the positions and bounding boxes of ball and players (\autoref{fig:system} A-1), detecting actions from the data (\autoref{fig:system} A-2), classifying tactics (\autoref{fig:system} A-3), and generating reasonable outputs from large language model (LLM) (\autoref{fig:system} B-1). \ourtool{} generates the embedded visualization (\autoref{fig:system} (B-3)) based on data from \autoref{fig:system} (A-1 and 2). 


Our solution is to pre-process all data that need to produce the explanation by using computer vision pipeline and make those data to textual information that easily adopt to current LLM. 
To do this, we utilize prior research~\cite{chen2023iball} that includes datasets tracking the bounding boxes of both the ball and players. The dataset has the bounding boxes ball and players every frame. The ball owner is calculated by the closest player with ball. We utilize x and y position in court from the SportVU \cite{SportVU24} to classify tactics and recognize which player is in one-on-one relationship or defending to detect the actions.

\subsubsection{Action Detection}
\begin{figure}[h]
\centering
\includegraphics[width=0.5\textwidth]{figs/action_graph.png}
\caption{An action list displays the series of actions performed by offensive players, including Pass, Cut, Screen, and Shoot. The main actions are identified based on ball movement or movements that enhance scoring opportunities, such as Shoot or Pass the ball. To extract the main actions related to Pass and Shoot, we establish criteria to filter out the less significant actions between Cuts and Screens.}
\label{fig:action_graph}
\end{figure}

Detecting actions from players' movements in the video plays an important role in explaining strategies and in-game decisions and satisfying the requirement (R2). A strategy consists of a series of actions, which are players' movements, such as a screen, a pass, and a cut \cite{sicilia2019deephoops}. As shown in \autoref{fig:system} (A-2), we define four different actions: the screen, the pass, the cut, and the shoot, as follows:
\begin{itemize}
    \item \textbf{Screen}: Player A attempts to block or delay a defender to create space and time for moving to a better position for offense or a shot \cite{tian2019use}. More technically, an offensive player performs a screen on a defender who is marking another offensive player with the ball at a close distance. We compute the \textit{distances} among players to check offensive players are close to defensive players and identify offensive players who change their one-on-one relationship.
    \item \textbf{Pass}: Player A sends the ball to his teammate B, who has a higher chance of scoring at the basket. We detect the pass by observing changes in the \textit{ball owner} within the same team, checking every frame.
    \item \textbf{Cut}: A cut is performed by a player without possession of the ball. The player moves from one location to another on the court to create space or move away from a defender, aiming for better offensive opportunities \cite{courel2018inside, tian2019use}. Since it is easier for a defender to guard a stationary offensive player, the offensive player moves quickly to another region to evade defense. We divide the court into 10 sub-regions, such as key, post, wing, etc., \cite{unkown10glossary}, and detect offensive players who move at 6 feet per second speed \cite{Wu2022OBTrackerVA} to a different area.    
    \item \textbf{Shoot}: A shot marks the end of an offense, and possession will change whether the player makes or misses the points. We detect changes in ball possessions between the two teams.
\end{itemize}

Another important aspect is the extraction of significant actions, since many different actions will be captured by our above criteria.
The redundant ones that are not crucial to strategies lead to degrade the user experience to show all actions. One solution is to choose important actions. The pass is the most significant factors to deploy strategies, and shooting is an essential part of scoring points in basketball \cite{tian2019use}. As shown in \autoref{fig:action_graph}, we identify the main actions as pass and shoot, while the other actions such as cut and screen can be sub actions, since some irrelevant or less important cuts and screens disrupt the explanation of the strategy. We build an action list to filter out irrelevant actions. We filter out that the cuts do not directly affect receiving a pass, while the screens do not aid players who have the ball or will receive the ball based on distance between the players and screen position. For example, one player cannot receive the ball from the cut in \autoref{fig:action_graph} (1), then the cut is disconnected. Similarly, the screen in \autoref{fig:action_graph} (2) is performed but does not have a huge impact to proceed play and disconnected and excluded based on distance between screen position and previous and next passes. The outputs of action detection are action type with frame index and the coordinates of players.

% in game decision

\subsubsection{Tactic Detection}
To classify tactics, we take players' coordinate data (e.g,. x and y position on the court) from SportVU \cite{SportVU24} and predict the label of tactics, as shown in \autoref{fig:system} (A-3).
To build a classifier model, we utilize data for the movement of players that match with specific tactics \cite{tsai2017recognizing}. The data includes x and y coordinates of each individual player on the courts as normalized values, along with the tactic label such as Back-Side Pick and Roll, Elevator, Pin-Down, etc. It consist of only 134 tactics in total, making it challenging to apply deep learning or complex models. A K-Nearest Neighbors (KNN) algorithm is a reasonable solution \cite{tian2019use} since it is able to identify a K number of similar data points based on its distance metrics (e.g., Euclidean distance.) We trained this algorithm using the existing tactic data \cite{tsai2017recognizing} to predict tactic label for the new input data. Another important aspect is that we use fastDTW \cite{salvador2007toward}, a refined version of Dynamic Time Warping (DTW) that is optimized linear and time and space complexity. The DTW is a method used to calculate the similarity between two time series, allowing one of the series to be non-linearly adjusted by expanding or compressing its timeline. This adjustment is crucial to match the difference lengths clips for computing the similarity between data, since the duration of clips vary. After classifying tactic, the information tactic will be provided to LLM.






%although important for the successful execution of a team’s game plan, are rarely evaluated. Even when we have volume
%statistics from these actions, the context is usually absent, which makes it hard to evaluate the importance of each of these
%actions. For example, simply counting passes can be very misleading; a pass exchange in the backcourt is certainly not as valuable as a pass that leads to an open three point shot.



==> sections/backup/5vis_v1.tex <==
\begin{figure}[ht]
    \includegraphics[width=0.5\textwidth]{figs/pass_iter.png}
    \includegraphics[width=.25\textwidth]{figs/cut_iter.png} \hfill
    \includegraphics[width=.25\textwidth]{figs/screen_iter.png}
     
    \caption{The iteration design process to design action visualizations (i.e., Pass, Cut, and Screen). From P1 to P4, we remove the occlusion and highlight the two players who send and receive the ball. For the cut, we indicate the exact location that a player will move with flash-forward animation from C1 to C2, while the screen demonstrate a wall to be easily identified a player set on screen from S1 to S2.}
    \label{figs:iter}
\end{figure}


\section{Visualization}
Drawing on our design requirements in Sec. 3, we design a series of visualizations and user interfaces. Our first requirement (interaction for complex questions, R1) does not necessarily require a response in the form of visualization, since the answer can be provided as simple textual information. We focus on the second and third design requirements to address strategic and in-game decision-making questions (R2), and to facilitate storytelling from the different narrative perspectives (R3).

\subsection{Action based Visualization}
To meet the requirement (R2 - the strategic and in-game decision questions), we present three different action based visualizations in terms of Pass, Cut, and Screen. Since the a complex series of actions cannot understand while playing video, we demonstrate the visualizations while stopping the video play in specific frames that includes actions. The data that need to visualize is generated by \autoref{fig:system} (A-1 and 2), including players' coordinate, bounding boxes, and frames.



% \begin{figure*}
%     \includegraphics[width=.33\textwidth]{figs/pass.png}\hfill
%     \includegraphics[width=.33\textwidth]{figs/cut.png}\hfill
%     \includegraphics[width=.33\textwidth]{figs/screen.png}
%     \caption{}
% \end{figure*}

\begin{figure*}
    \includegraphics[width=1.0\textwidth]{figs/perspective.png}
    \caption{The figure (A) shows the third person perspective narrative like commentaries, whereas the figure (B) demonstrates the first person perspective by integrating the action visualizations and narratives around the players to make people more engaged and immersive.}
    \label{figs:perspective}
\end{figure*}

\subsubsection{\textbf{Pass} Visualization Design Iteration}
The purpose of a pass is to send the ball to another player form the same team who has a higher chance of scoring at the basket. Our main visualization goal is to highlight the players who send and receive the ball, as well as the direction of the ball. As shown in \autoref{figs:iter} (P4), we finalize our pass visualization with circles on the two players who send and receive the ball, an arrow that indicates the direction of the ball and is located below the players to avoid occlusions, and add a flash-forward effect to show the next movement of the players. The circles and arrow are rotating around the players and showing the trajectories from the sender to the receiver, respectively. To design our final visualization, we iterate our designs from \autoref{figs:iter} from P1 to P4. Initially, we visualized the basic arrow that shows the change of ball possession and direction like \autoref{figs:iter} (P1). However, this P1 approach obscures the player, which make it difficult to understand the actions of the two players and the direction of the ball. To avoid the occlusion, we decide to draw the arrow below the players and cover the players once more after drawing the arrow like prior work \cite{chen2023iball}, as shown in \autoref{figs:iter} (P2). The current P2 design has a problem when there are many players around the receiver while passing. The second iteration is to represent circles at the bottom of the players to highlight them and tighten the visualization, helping fans recognize the important players. The last iteration from P3 to P4 is design to help fans easily identify the visualization, supporting the animations of circles and arrows, giving a flash-forward effect to show the next few future steps, and providing additional colors to enable fans to distinguish the visualization easily. We choose the colors based on each individual team colors, which can easily be distinguished by the team's fans.

\subsubsection{\textbf{Cut} Visualization Design Iteration}
The objective of a cut is that a player who does not hold the ball moves from one region to another one on the court. This movement is performed for having space or distance from a defender, seeking improved attacking positions to score  \cite{courel2018inside, tian2019use}. Our final cut visualization shows the direction of the players using arrows and demonstrates their specific movement to locations with area visualization, as shown in \autoref{figs:iter} (C2). Another important aspect in cut visualization is to preview the trajectories that the player takes. We present a flash-forward to preview the action before the player makes their move. In the \autoref{figs:iter} (C2), the player in blue dashed line illustrates before cut, while the green line present after cut to show the movement. Our visualization aims to highlight the movement and direction of the player. We refine the cut visualization design from C1 to C2, similar to how we evolved designs from P1 to P4, but we omit the details of the entire iteration process here. The C1 in \autoref{figs:iter} displays the visualization of the cut with only an arrow visualization, showing only the direction of the player. However, an arrow is insufficient to accurately represent the exact future location of the player and trace the trajectories. Therefore, we design the C2 visualization design with the arrow, the area representation, and flash-forward effect to enhance the depiction.

\subsubsection{\textbf{Screen} Visualization Design Iteration}
The screen aims to obstruct or slow down a defender to create space and time, enabling team players who hold the ball to move to a better position, dribble, or take a shot \cite{tian2019use}. We design our screen visualization to help fans identify which offensive player performs a screen on a defender. Our screen visualization is designed with an arrow and a screen wall to indicate the two different players and where the offensive player performs the screen, as shown in \autoref{figs:iter} (S2). \autoref{figs:iter} (S1) shows our initial design of the screen visualization, allowing fans to see only the arrow. However, identifying the screen action is challenging due to confusion among different actions as well as the presence of many players. We finalize our screen visualization (S2) after iterating our design, similar to the pass action \autoref{figs:iter} (P1-P4).


\subsection{Narrative and Visualization Integration}

To satisfy our design requirement (R3 - Storytelling combining narrative and visualization), we integrate narratives and visualizations for an effective and intuitive presentation. \autoref{figs:perspective} demonstrates the exact same situation that Stephen Curry pass to Andre Iguodala with different person perspectives. One important aspect of storytelling is person perspectives (e.g., third and first-person perspectives) that change user experiences. In basketball games, the third-person perspective allows for a more analytical and comprehensive view of the game, while the first-person view creates a more immersive experience for the fans, making them feel closer to the action. The third-person perspective is a common way to explain basketball plays, like a commentator's description (e.g., \textit{"Andre Iguodala cuts from the post to the wing to space the floor..."}), as shown in \autoref{figs:perspective} (A). This perspective can easily be integrated into a visualization with one chatbox, which does not require any additional interfaces. However, fans are confused and distracted with the traditional chatbox in the first-person perspective since the players express their emotions and thoughts, and call other team players by name (e.g., \textit{"Perfect timing, Andre. Cutting towards the high post to create a mismatch..."}). Using a conventional chatbot can lead to misunderstandings and make it hard to follow interactions between players. We present a new user interface for the first-person perspective to integrate the narrative and visualization at the top or bottom of the players to indicate who is talking, as demonstrated in \autoref{figs:perspective} (B). In \autoref{figs:perspective} (B), the integrated chatbox follows around a player while playing video and shows the interface that allows manipulation of players' conversations by clicking prev, play, and next.

==> sections/backup/5vis_v2.tex <==
\begin{figure}[ht]
    \includegraphics[width=0.5\textwidth]{figs/iter.png}
    % \includegraphics[width=.25\textwidth]{figs/cut_iter.png} \hfill
    % \includegraphics[width=.25\textwidth]{figs/screen_iter.png}
     
    \caption{The iteration design process to design action visualizations (i.e., Pass, Cut, and Screen). From P1 to P4, we remove the occlusion and highlight the two players who send and receive the ball. For the cut, we indicate the exact location that a player will move with flash-forward animation from C1 to C2, while the screen demonstrate a wall to be easily identified a player set on screen from S1 to S2.}
    \label{figs:iter}
\end{figure}

\section{Visualization}
% Drawing on our design requirements in Sec. 3, we design a series of visualizations and user interfaces. 
% Our first requirement (interaction for complex questions, R1) does not necessarily require a response in the form of visualization, since the answer can be provided as simple textual information. 
% We focus on the second and third design requirements to address strategic and in-game decision-making questions (R2), and to facilitate storytelling from the different narrative perspectives (R3).

According to R3, we aim to visualize the explanations into the videos.
We achieve this by \zt{xxx}.

\subsection{Visualizing Actions}
To meet the requirement (R2 - the tactical and in-game decision questions), 
we present three embedded visualizations for Pass, Cut, and Screen.
Since the a complex series of actions cannot understand while playing video, 
we demonstrate the visualizations while stopping the video play in specific frames that includes actions. 
The data that need to visualize is generated by~\autoref{fig:system} (A-1 and 2), 
including players' coordinate, bounding boxes, and frames.

% \begin{figure*}
%     \includegraphics[width=.33\textwidth]{figs/pass.png}\hfill
%     \includegraphics[width=.33\textwidth]{figs/cut.png}\hfill
%     \includegraphics[width=.33\textwidth]{figs/screen.png}
%     \caption{}
% \end{figure*}

\begin{figure*}
    \includegraphics[width=1.0\textwidth]{figs/perspective.png}
    \caption{The figure (A) shows the third person perspective narrative like commentaries, whereas the figure (B) demonstrates the first person perspective by integrating the action visualizations and narratives around the players to make people more engaged and immersive.}
    \label{figs:perspective}
\end{figure*}

\subsubsection{Visualizing a \Pass{}}
% The goal of a \textsc{Pass} in basketball is to transfer the ball to a teammate who is in a better position to score.
To visualize a \Pass{}, we aim to clearly delineate the dynamics of passing by highlighting the players involved in the pass—the sender and receiver—along with the ball's trajectory.
As demonstrated in~\autoref{figs:iter} P4, 
our visual design employs two rotating circles that mark the sender and receiver, respectively, and an arrow beneath the players to indicate the ball's passing direction. %, thus avoiding occluding the scene.
Additionally, we incorporate a flash-forward effect~\cite{} to preview the players' subsequent movements.

The development of our visual design was an iterative process, detailed in~\autoref{figs:iter} 
 P1 to P4. 
Initially, we used a basic arrow to signify the change in ball possession and its direction (P1), but this approach proved problematic as it occludes the players.
To counter this, we repositioned the arrow beneath the players on the court (\autoref{figs:iter} P2).
However, the P2 design encountered visibility issues in crowded scenes.
Our subsequent iterations focused on enhancing visibility and understanding: 
we introduced circles beneath the players to emphasize their roles (P3) and further refined the design (P4) by animating the circles and arrow and adding a flash-forward effect for future movements, and employing team-specific colors for easy identification. 
This iterative approach, culminating in our final design, facilitates an intuitive and engaging visualization for fans to understand a \Pass{} action.

% , allowing them to follow the pass dynamics seamlessly, even amidst the fast-paced action on the court.
% , drawing on previous studies for inspiration (Chen et al., 2023), as seen in P2. 
% The visualization dynamically depicts the ball's path from sender to receiver with rotating circles and arrows, tracing their trajectory. 
% Our main visualization goal is to highlight the players who send and receive the ball, 
% as well as the direction of the ball. 
% As shown in~\autoref{figs:iter}P4, 
% we finalize our pass visualization with circles on the two players who send and receive the ball, an arrow that indicates the direction of the ball and is located below the players to avoid occlusions, and add a flash-forward effect to show the next movement of the players. 

% The circles and arrow are rotating around the players and showing the trajectories from the sender to the receiver, respectively. 
% To design our final visualization, we iterate our designs (i.e., P1 to P4 in \autoref{figs:iter}). 
% Initially, we visualized the basic arrow that shows the change of ball possession and direction like \autoref{figs:iter} (P1). However, this P1 approach obscures the player, which make it difficult to understand the actions of the two players and the direction of the ball. To avoid the occlusion, we decide to draw the arrow below the players and cover the players once more after drawing the arrow like prior work \cite{chen2023iball}, as shown in \autoref{figs:iter} (P2). The current P2 design has a problem when there are many players around the receiver while passing. 
% The second iteration is to represent circles at the bottom of the players to highlight them and tighten the visualization, helping fans recognize the important players. The last iteration from P3 to P4 is design to help fans easily identify the visualization, supporting the animations of circles and arrows, giving a flash-forward effect to show the next few future steps, and providing additional colors to enable fans to distinguish the visualization easily. We choose the colors based on each individual team colors, which can easily be distinguished by the team's fans.


\subsubsection{Visualizing a \Cut{}}
The purpose of a \Cut{} in basketball is for a player without the ball to move from one part of the court to another, aiming to create space from defenders and find better positions for shooting~\cite{courel2018inside, tian2019use}.
We visualize a \Cut{} by using an arrow to indicate the player's movement direction 
and an area visualization to demonstrate the specific court locations they are moving into (\autoref{figs:iter} C2).
Particularly, we incorporate a flash-forward effect~\cite{},
which previews the player's trajectory before the actual movement occurs. 
In \autoref{figs:iter} C2, a blue dashed line represents the player's position before the cut, and a green line indicates the position after the cut, effectively showcasing the movement path.
% A key feature of our cut visualization is the 
% inclusion of a , 

Our approach to visualizing a \Cut{} was also iteratively refined.
The initial design (\autoref{figs:iter} C1) depicted a \Cut{} with a simple arrow, highlighting the player’s direction but failing to convey the precise future location or the movement trajectory. 
To address these limitations, the refined design (\autoref{figs:iter} C2) integrates the arrow with area representation and the flash-forward effect.
This enhancement not only clarifies the direction and intent behind a player's \Cut{} but also provides viewers with a predictive insight into the player's positioning, 
enriching the overall understanding of the game’s dynamics.


\subsubsection{Visualizing a \Screen{}}
A \Screen{} in basketball is executed to impede or slow a defender, thereby creating space and time for the offensive players. 
This allows the player with the ball to either move into a more advantageous position, dribble past opponents, or take a shot~\cite{tian2019use}. 
To visualize a \Screen{}, we aim to enable fans to easily identify when and by whom a screen is set against a defender
As shown in \autoref{figs:iter} S2, our design incorporates both an arrow and a depiction of a screen wall. 
This combination clearly distinguishes the involved players and the location where the screen occurs.

The initial design (\autoref{figs:iter} S1) utilized an arrow to indicate the screen action. 
However, this approach proved insufficient for clear identification, as it often blended with other actions and occluded by the presence of multiple players on the court. 
We thus improved it and concluded to the current design, which ensuring that fans can easily recognize and understand this crucial aspect of a \Screen{}

\subsection{Narrative and Visualization Integration}
\zt{zt will come back later after refining Sec3}
To satisfy our design requirement, we integrate narratives and visualizations for an effective and intuitive presentation. \autoref{figs:perspective} demonstrates the exact same situation that Stephen Curry pass to Andre Iguodala with different person perspectives. 
One important aspect of storytelling is person perspectives (e.g., third and first-person perspectives) that change user experiences. In basketball games, the third-person perspective allows for a more analytical and comprehensive view of the game, while the first-person view creates a more immersive experience for the fans, making them feel closer to the action. The third-person perspective is a common way to explain basketball plays, like a commentator's description (e.g., \textit{"Andre Iguodala cuts from the post to the wing to space the floor..."}), as shown in \autoref{figs:perspective} (A). This perspective can easily be integrated into a visualization with one chatbox, which does not require any additional interfaces. However, fans are confused and distracted with the traditional chatbox in the first-person perspective since the players express their emotions and thoughts, and call other team players by name (e.g., \textit{"Perfect timing, Andre. Cutting towards the high post to create a mismatch..."}). Using a conventional chatbot can lead to misunderstandings and make it hard to follow interactions between players. We present a new user interface for the first-person perspective to integrate the narrative and visualization at the top or bottom of the players to indicate who is talking, as demonstrated in \autoref{figs:perspective} (B). In \autoref{figs:perspective} (B), the integrated chatbox follows around a player while playing video and shows the interface that allows manipulation of players' conversations by clicking prev, play, and next.
